{\sc mirkwood:} Fast and Accurate SED Modeling Using Machine Learning

Traditional spectral energy distribution (SED) fitting codes used to derive galaxy physical properties are often uncertain at the factor of a few level owing to uncertainties in galaxy star formation histories and dust attenuation curves. Beyond this, Bayesian fitting (which is typically used in SED fitting software) is an intrinsically compute-intensive task, often requiring access to expensive hardware for long periods of time. To overcome these shortcomings, we have developed {\sc mirkwood}: a user-friendly tool comprising of an ensemble of supervised machine learning-based models capable of non-linearly mapping galaxy fluxes to their properties. By stacking multiple models, we marginalize against any individual model's poor performance in a given region of the parameter space. We demonstrate \textsc{mirkwood}'s significantly improved performance over traditional techniques by training it on a combined data set of mock photometry of z=0 galaxies from the \textsc{Simba}, \textsc{EAGLE} and \textsc{IllustrisTNG} cosmological simulations, and comparing the derived results with those obtained from traditional SED fitting techniques. \textsc{mirkwood} is also able to account for uncertainties arising both from intrinsic noise in observations, and from finite training data and incorrect modeling assumptions. To increase the added value to the observational community, we use Shapley value explanations (SHAP) to fairly evaluate the relative importance of different bands to understand why particular predictions were reached. We envisage \textsc{mirkwood} to be an evolving, open-source framework that will provide highly accurate physical properties from observations of galaxies as compared to traditional SED fitting.

==> ABSTRACT.tex <==
Bayesian codes are routinely used to fit observed photometries with underlying models of star formation, evolution, and dust attenuation. However, results based on hydrodynamical simulations have exposed biases in these methods at a factor of a few in the derived physical properties. Furthermore, Bayesian fitting is an intrinsically compute-intensive task, often requiring access to expensive hardware for long periods of time. To overcome these shortcomings, we have developed {\sc mirkwood}: a user-friendly tool comprising of an ensemble of supervised machine learning-based models capable of non-linearly mapping galaxy fluxes to their properties. By stacking multiple models, we marginalize against any individual model's poor performance in a given region of the parameter space. We demonstrate \textsc{mirkwood}'s superior performance by training it on a combined data set of mock photometry from z=0 and z=2 galaxies from the \textsc{Simba}, \textsc{EAGLE} and \textsc{IllustrisTNG} simulations, and comparing the derived results with those obtained from traditional SED fitting techniques. \textsc{mirkwood} is also able to account for uncertainties arising both from missing observations in informative bands and intrinsic noise in observations, and from finite training data and incorrect modeling assumptions. To increase the added value to the observational community, we use Shapley value explanations (SHAP) to fairly evaluate the relative importance of different bands to understand why particular predictions were reached. We envisage \textsc{mirkwood} to be an evolving, open-source framework that will provide highly accurate physical properties from observations of galaxies as compared to traditional SED fitting.

==> CONCLUSION.tex <==
\section{Conslusion}\label{sec:conclusion}


==> DATA.tex <==
\section{Training on Cosmological Galaxy Formation Simulations}\label{sec:data}

The first step in a supervised ML code is to train the software on known results.  To do this, we employ three state-of-the-art cosmological galaxy formation simulations where we know the true physical properties.  We then generate mock SEDs from the galaxies in these simulations using stellar population synthesis models and dust radiative transfer; these mock SEDs allow our ML algorithms to develop a highly accurate mapping between input photometry and galaxy physical properties.

We train on a set of three galaxy formation simulations: {\sc Simba} \citep{dave_simba}, {\sc Eagle} \citep{schaye_2015_eagle,schaller_2015_eagle,mcalpine_2016_eagle_cat}, and {\sc IllustrisTNG} \citep{vogelsberger2014introducingillustris}. These models provide a large and diverse sample of galaxies with realistic growth histories, and free us from being dependent on any one set of galaxy model assumptions. In the following subsections, we describe each simulation and the galaxy formation models included in each suite as well as our galaxy selection method and computational techniques for generating mock SEDs for each galaxy. 

\subsection{Cosmological Galaxy Formation Simulations}\label{sec:data_sims}

\textbf{\textsc{Simba}} \citep{dave_simba}: The {\sc Simba} galaxy formation model is a descendent of the {\sc Mufasa} model, and uses the {\sc Gizmo} gravity and hydrodynamics code \citep{hopkins_2015_gizmo}. {\sc Simba} uses an H$_2$-based star formation rate (SFR), given by the density of H$_2$ divided by the local dynamical timescale. The H$_2$ density itself relies on the metallicity and local column density \citep{krumholz2014despotic}. The chemical enrichment model tracks $11$ elements from from Type II supernovae (SNe), Type Ia SNe, and asymptotic giant branch (AGB) stars with yields following \cite{nomoto_simba_sne_yields}, \cite{iwamoto_1999_sne_yields}, and \cite{Oppenheimer_2006_agb_yields}, respectively. Sub-resolution models for stellar feedback include contributions from Type II SNe, radiation pressure, and stellar winds. The two-component stellar winds adopt the mass-loading factor scaling from {\sc fire} \citep{angles-alcazar_FIRE} with wind velocities given by \cite{muratov_2015}. Metal-loaded winds are also included, which extract metals from nearby particles to represent the local enrichment by the SNe driving the wind. Feedback via active galactic nuclei (AGN) is implemented as a two-phase jet (high accretion rate ) and radiative (low accretion rate) model, similar to the model used in {\sc IllustrisTNG} described below. Finally, dust is modeled self-consistently, produced by condensation of metals ejected from SNe and AGB stars, and is allowed to grow and erode depending on temperature, gas density, and shocks from local Type II SNe \citep{li2018dark}. The tunable parameters in {\sc Simba} were chosen to reproduce the M$_{BH}$-$\sigma$ relation and the galaxy stellar mass function (SMF) at redshift z $=0$. For our analysis, we use a box with $25/h$ Mpc side length with $512^3$ particles, resulting in a baryon mass resolution of $1.4\times$ $10^6 \: \mathrm{M}_{\odot}$. 
    

\textbf{Eagle} \citep{crain_2015_eagle, schaye_2015_eagle, schaller_2015_eagle, mcalpine_2016_eagle_cat}: The Evolution and Assembly of GaLaxies and their Environments ({\sc eagle}) suite of cosmological simulations is based on a modified version of the smoothed particle hydrodynamics (SPH) code {\sc gadget} 3 \citep{springel_2005_gadget}. Star formation occurs via gas particles that are converted into star particles at a rate that is pressure dependent and gas temperature and density limited, following \cite{schaye_2004_eagle_sfr} and \cite{schaye_dallavecchia_2008_eagle_sfr}. The chemical enrichment model tracks $9$ independent elements generated via winds from AGB stars, winds from massive stars, and Type II SNe following \cite{Wiersma_2009_eagle_yields}, \cite{Portinari_1998_eagle_yields}, and \cite{Marigo_2001_eagle_yields}, respectively. Stellar feedback from Type II SNe heats the local ISM, delivering fixed jumps in temperature and a fraction of energy from the SNE, and similarly, a single feedback mode for AGN injects thermal energy proportional to the BH accretion rate at a fixed efficiency into the surrounding gas. Like {\sc simba}, the parameters in {\sc eagle} have been tuned to reproduce the z $=0.1$ galaxy SMF. For our analysis, we use a $50/h$ Mpc box size with $752^3$ particles, resulting in a baryon mass resolution of $1.81\times$ $10^6 \: \mathrm{M}_{\odot}$. 
    

\textbf{IllustrisTNG} \citep{weinberger_2017_tng, pillepich_2018_tng1, pillepich_2018_tng2}: {\sc IllustrisTNG} is an updated version of the {\sc illustris} project, based on the {\sc arepo} \citep{springel_2010_arepo} magneto-hydrodynamics code. Star formation occurs in gas above a given density threshold, at a rate following the Kennicutt-Schmidt relation \citep{schmidt_1959_sfr, kennicutt_1989_sfr}. As stars evolve and die, nine elements are tracked via enrichment from Type II SNe and AGB stars following the models and yields of \cite{Wiersma_2009_eagle_yields}, \cite{Portinari_1998_eagle_yields}, and \cite{nomoto_simba_sne_yields}. Star formation also drives galactic scale winds. These hydrodynamically decoupled wind particles are injected isotropically with an initial speed that scales with the the local 1D dark matter velocity dispersion. The galactic winds carry additional thermal energy to avoid spurious artifacts where the wind particles hydrodynamically recouple with the gas. Like {\sc simba}, {\sc IllustrisTNG} features a two-mode feedback model for AGN: thermal energy is injected into the surrounding ISM at high accretion rates, while BH-driven winds are produced at low accretion rates. Tunable parameters were chosen in {\sc IllustrisTNG} to match observations including the SFM, the star formation rate density, and the stellar mass-halo mass relation at z $=0$. We use the TNG100 box with a baryonic mass resolution of $1.4\times$ $10^6 \: \mathrm{M}_{\odot}$. 

\subsection{Galaxy Selection}\label{sec:data_galaxyselection}
Galaxies from each simulation were identified with their respective friends-of-friends (FOF) algorithms. We use the publicly available galaxy catalogues for {\sc eagle} \citep{mcalpine_2016_eagle_cat} and {\sc IllustrisTNG} \citep{nelson_tng_cat} in which subhalo structures are identified by a minimum of 32 particles with the {\sc subfind} algorithm \citep{springel_2001_subfind, dolag_2009_subfind}. For {\sc simba}, we have employed  {\sc caesar}\footnote{https://github.com/dnarayanan/caesar} \citep{caesar}, which identifies halos and galaxies in snapshots based on the number of bound stellar particles (a minimum of 32 particles defines a galaxy). To ensure our galaxy sample is robust across the three simulations, we select galaxies from the full subhalo populations that have (i) a stellar mass above the minimum mass found in the z $=0$ {\sc simba} snapshot ($4.4\times$ $10^7 \: \mathrm{M}_{\odot}$) and (ii) have a nonzero gas mass. Due to computational limits, we randomly sample 10,000 galaxies from the $\sim$85,000 previously identified {\sc IllustrisTNG} galaxy sample, though we ensure that this subsample matches the intrinsic SFM of the entire sample. After these selections, we have a total of $1797$, $4697$, and $10000$ from the {\sc Simba}, {\sc Eagle}, and {\sc IllustrisTNG} simulations respectively for redshift $z=0$. For redshift $z=2$, an additional $17,020$ galaxies are included in the training set. 


\subsection{Mock SEDs from 3D Radiative Transfer}\label{sec:data_radiativetransfer}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{pd_pipeline.pdf}
    \caption{Data pipeline for each simulated galaxy. Once galaxies are selected from each simulation, we perform 3D dust radiative transfer with {\sc powderday}, which utilizes {\sc fsps} to generate the stellar SEDs and {\sc hyperion} to propagate the stellar SEDs through a dusty medium dependent. We then sample mock photometry in $33$ filters from the {\sc powderday} SED.} 
    \label{fig:pd_sed}
\end{figure*}

Our analysis relies on realistic galaxy SEDs as input to predict physical properties including stellar mass and SFR. To produce these SEDs, we perform full 3D dust radiative transfer (RT) for each galaxy in our subsamples. We use the radiative transfer code {\sc powderday}\footnote{https://github.com/dnarayanan/powderday} \citep{pd_2020} to construct the synthetic SEDs by first generating with {\sc fsps} \citep{fsps_1, fsps_2} the dust free SEDs for the star particles within each cell using the stellar ages and metallicities as returned from the cosmological simulations. For these, we assume a \cite{kroupa_initial_2002} stellar IMF and the {\sc mist} stellar isochrones \citep{mist_1, mist_2}. These {\sc fsps} stellar SEDs are then propagated through the dusty ISM. Here, differences in the RT model arise as dust is implemented differently in each simulation. {\sc eagle} and {\sc IllustrisTNG} do not have a native dust model and so we assume a constant dust mass to metals mass ratio of $0.4$ \green{\citep{dwek_1998_dust_to_metals, vladilo_1998_dust_to_metals, watson_2011_dust_to_metals}}. For {\sc simba}, the diffuse dust content is derived from the on-the-fly self-consistent model of \cite{qi_dust}. From there, the dust is treated identically between simulations: it is assumed to have extinction properties following the carbonaceous and silicate mix of \cite{draine_infrared_2007}, that follows the \cite{weingartner_draine} size distribution and the \cite{draine_03} renormalization relative to hydrogen. We assume $R_{\rm V} \equiv A_{\rm V}/E(B-V) = 3.15$. We do not assume further extinction from sub-resolution birth clouds. Polycyclic aromatic hydrocarbons (PAHs) are included following the \citet{robitaille_pahs} model in which PAHs are assumed to occupy a constant fraction of the dust mass (here, modeled as grains with size $a<20$ \AA) and occupying $5.86\%$ of the dust mass. The dust emissivities follow the \citet{draine_infrared_2007} model, though are parameterized in terms of the mean intensity absorbed by grains, rather than the average interstellar radiation field as in the original Draine \& Li model. The radiative transfer propagates through the dusty ISM in a Monte Carlo fashion following the \cite{lucy_rt} algorithm, in order to determine the equilibrium dust temperature in each cell. We iterate until the energy absorbed by $99\%$ of the cells has changed by less than $1\%$.  Note, a result of these calculations is that while we assume the \cite{draine_infrared_2007} extinction curve in every cell, the effective {\it attenuation} curve is a function of the star-dust geometry, and therefore varies from galaxy to galaxy \citep{attenuation_araa}.


The result of the {\sc powderday} radiative transfer is the UV - FIR spectrum for each galaxy. From there, we sample broadband photometry in $33$ filters, ensuring robust SED coverage. These filters are shown in Table \ref{table:filters}. Our training set for {\sc mirkwood} includes photometry at signal-to-noise ratios (SNR) of 2, 10, and 20.  

\input{filters_table_long}

\subsection{Prospector SED Fitting}\label{sec:data_prospector}

We compare our results from {\sc mirkwood} to traditional galaxy SED fitting using the state-of-the-art SED fitting code, {\sc Prospector} \citep{2019ascl.soft05025J, leja_deriving_2017, leja_how_2019}\footnote{https://github.com/bd-j/prospector}. {\sc Prospector} wraps {\sc fsps} stellar modeling with {\sc dynesty} \citep{dynesty} Bayesian inference to provide estimates of galaxy properties given models forms for the galaxy star formation history (SFH), metallicity, and dust content. For the galaxy SFH, we use the nonparametric linear piece-wise function as described in \cite{leja_how_2019} with 6 time bins spaced equally in logarithmic time. The stellar metallicity is tied to the inferred stellar mass of the galaxy, constrained by the \cite{gallazzi_ages_2005} M*-Z relation from SDSS DR7 data. The dust attenuation model follows \cite{kc_law}, in which the strength of the 2175 \AA \ bump is tied to the powerlaw slope. Dust emission follows the \cite{draine_infrared_2007} model. Prior distributions for model components approximately follow those outlined in \cite{lower_stellar_mass} and have been shown to reasonably reproduce {\sc simba} galaxy properties including stellar mass and SFR. 

We provide the same mock {\sc powderday} broadband SEDs to {\sc prospector} as {\sc mirkwood} with the same SNRs. In all comparisons to {\sc mirkwood}, we report the median value of the posterior distribution from the {\sc prospector} fit for each galaxy property. 


\begin{table*}
    \caption{Summary statistics of the five galaxy properties in this paper, for all three hydrodynamical simulations. Each tuple consists of value at z=0 and value at z=2, from left to right respectively.}
    \label{tab:datasetsummary}
    \centering
    \begin{tabular}{ccccc}
    \toprule
     & & {\sc Simba} &  {\sc Eagle} &  {\sc IllustrisTNG} \\ \tableline
     & Min & (0.0, 2.0)  &  (0.0, 2.0) &  (0.0, 2.0) \\
     & Max & (0.0, 2.0)  &  (0.0, 2.0) &  (0.0, 2.0) \\
    $z$ & Mean & (0.0, 2.0)  &  (0.0, 2.0) &  (0.0, 2.0) \\
     & Median & (0.0, 2.0)  &  (0.0, 2.0) &  (0.0, 2.0) \\
     & Std.Dev. & (0.0, 0.0)  &  (0.0, 2.0) &  (0.0, 0.0) \\ \tableline
     & Min & (7.64, 7.70)  &  (7.64, 7.64) &  (7.70, 6.06) \\
     & Max & (12.15, 11.63)  &  (12.01, 11.01) &  (12.19, 11.46) \\
    $\log_{10}(\frac{\rm{M}^{\star}}{\rm{M}_{\odot}})$ & Mean & (8.91, 8.37)  &  (8.71, 8.31) &  (8.82, 6.75) \\
     & Median & (8.78, 8.16)  &  (8.50, 8.13) &  (8.65, 6.41) \\
     & Std.Dev. & (0.86, 0.64)  &  (0.83, 0.60) &  (0.85, 0.82) \\ \tableline
     & Min & (0.0, 2.41)  &  (2.81, 4.40) &  (4.72, 5.66) \\
     & Max & (8.63, 8.99)  &  (10.5, 8.94) &  (10.26, 9.30) \\
    $\log_{10}(1+\frac{\rm{M}_{\rm{Dust}}}{\rm{M}_{\odot}})$ & Mean & (5.39, 4.81)  &  (6.25, 6.21) &  (6.82, 6.54) \\
     & Median & (5.33, 4.51)  &  (6.06, 6.05) &  (6.72, 6.39) \\
     & Std.Dev. & (1.47, 0.98)  &  (0.86, 0.64) &  (0.75, 0.56) \\ \tableline
     & Min & (-1.61, -1.69)  &  (-1.05, -1.67) &  (-1.27, 0.27) \\
     & Max & (0.08, 0.11)  &  (0.30, 0.35) &  (0.17, 0.52) \\
    $\log_{10}(\frac{\rm{Z}^{\star}}{\rm{Z}_{\odot}})$ & Mean & (-0.86, -1.2)  &  (-0.25, -0.80) &  (-0.49, 0.46) \\
     & Median & (-0.87, -1.24)  &  (-0.24, -0.80) &  (-0.50, 0.46) \\
     & Std.Dev. & (0.35, 0.24)  &  (0.18, 0.21) &  (0.28, 0.03) \\ \tableline
     & Min & (0.0, 0.0)  &  (0.0, 0.0) &  (0.0, 0.0) \\
     & Max & (1.35, 2.46)  &  (1.14, 1.84) &  (1.57, 0.16) \\
    $\log_{10}(1+\rm{SFR}_{100})$ & Mean & (0.10, 0.15)  &  (0.05, 0.14) &  (0.09, 0.00) \\
     & Median & (0.02, 0.03)  &  (0.01, 0.05) &  (0.03, 0.00) \\
     & Std.Dev. & (0.18, 0.31)  &  (0.11, 0.24) &  (0.15, 0.00) \\ \tableline
    \#Samples & & (1,797, 1,797) & (4,697, 4,697) & (10,073, 10,073) \\ \tableline 
    \end{tabular}
\end{table*}






==> DISCUSSION.tex <==
\section{Discussion and Future Work}\label{sec:discussion}
%https://arxiv.org/pdf/1905.08996.pdf
%To field-test {\sc mirkwood}, we plan to use it with data from the GAMA survey. This
Our work shows that it is possible to reproduce galaxy property measurements with high accuracy in a purely data-driven way by using robust ML algorithms that do not have any knowledge about the physics of galaxy formation or evolution. The biggest caveat here is that the training set must be closely representative of the data of interest, i.e. observations of real galaxies. We also demonstrate the necessity of carefully accounting for both the noise in the data and sparsity of the training set in any given parameter-space of interest. By combining galaxy simulations with disparate physics, we offer a way to better train our model for a real observation. Across all SNRs, we show a considerable improvement over state-of-the-art SED fitting using {\sc Prospector} and non-parametric SFH prior, both in terms of predictions and computing time. A notable result is that we are able to extract galaxy properties from photometries with SNRs as low as 5. We have also shown that it is possible to derive the redshift from purely photometric observations. All these contributions considered together imply indicate that scientifically interesting galaxy properties can be accurately and quickly measured on future datasets from large-scale photometric surveys.

Several avenues for future research remain open. The crux of our follow-up efforts will focus on development of {\sc mirkwood} to a higher level of complexity and precision. We identify the following areas for improvement:
\begin{enumerate}
    \item Extensive hyperparameter optimization: In this work we use {\sc NGBoost} models with hyperparameters marginally modified from the prescription of \cite{ren2019rongba_ngboost}. This is an easy avenue for gaining performance boost with respect to reconstruction of galaxy properties -- in future work we will leverage modern Bayesian hyperparameter optimization libraries to this end.
    \item Managing missing observations: Most real-life observations of galaxies do not contain observations in the same set of filters, nor is the SNR of the data in each filter the same. {\sc mirkwood} can easily accommodate both these complications, and in future work we will explore their impact on model performance.
    \item Synergistic spectroscopy: While spectroscopic data are considerably more expensive to obtain, there exist targets where photometry and spectra are available simultaneously \citep{carnall2019vandels}. Modeling both modes of data simultaneously can increase the SNR available to any model, and help significantly in reducing uncertainties in derived galaxy properties, thus enabling accurate re-construction of higher resolution ones such as a galaxy's entire star formation history. We will explore inclusion of a convolutional neural network to this end, similar to the work of \cite{lovell2019learning}.
    \item Probability calibration: This is a post-processing step that has been shown to improve predictions, measured both by deterministic and probabilistic metrics. ML algorithms are often over-confident, and unable to assess the degree of their fallacy -- if given a completely novel input, most commonly used ML algorithms are likely to predict a wrong label for it, instead of just saying, `I do not know the correct answer.' Probability calibration is widely used in the machine learning community \citep{measuring_calibration_in_deep_learning, probability_calibration1, crude_probability_calibration, lakshminarayanan_probability_calibration0}, albeit its adoption in astronomy has been slow.
    \item Randomized chaining: Here we have considered one particular way of chaining galaxy properties: redshift is considered when predicting stellar mass, redshift and stellar mass are considered when predicting dust mass, and so on all the way till SFR$_{100}$ (see Figure \ref{fig:chaining} for details). However, given the interdependence of all properties, a more justified approach would be to conside multiple such orderings and average the result. For instance, to predict stellar mass, $\rm{model}_1$ will be trained on just the galaxy fluxes, $\rm{model}_2$ on fluxes + redshift, $\rm{model}_3$ on fluxes + dustmass + SFR$_{100}$, and all such permutations. Finally, the predicted stellar mass results will be averaged.
    \item Redshift as input: It might very well be the case that for a given set of samples, high-confidence spectroscopic redshift is available, but photometry data is present only in a few bands. In such a case, it would be sensible to use redshift as an input rather than an output. We plan on upgrading our network so that {\sc mirkwood} can easily take a redshift as either a fixed input, or take a user-given prior for redshift which it will then aim to improve.
    \item Semi-supervised learning: In an effort to reduce the `domain gap' --  the difference between the training set(s) and real life data -- several semi-supervised algorithms have been developed and used. These can smoothly combine a computer simulated set of data with high-confidence real life-observations, such as spectra, to more closely approximate reality.
    \item Outlier detection and elimination: In its current implementation, {\sc mirkwood} is unable to identify and reject outlying inputs. These can result from any of the several data processing pipelines that are used to create scientifically interesting data products can fail and output nonsensical numbers, for example a flux absurdly high as $10^{252}$. This issue becomes even more urgent when dealing with semi-supervised learning, where data from real-life observations form part of the training set. In future we plan on exploring algorithms such as variational auto-encoders \citep{ghosh2016robust_variationalbayesianinference,zellner1988optimal_variationalbayesianinference} to this end.
\end{enumerate}

%that This allows for not only the use of semianalytic models as a training set for galaxy property measurement, but also a multiplication of template-fitting efforts–for example, if templatefitted stellar masses are available for a representative spectroscopic subset of a large photometric survey, then machine learning is a computationally efficient way to extend those template-fitting results to the larger photometric data set. As we have shown here, machine learning methods can learn even complicated relationships between galaxy properties and photometry measurements drawn from a small number of filters, indicating that scientifically interesting galaxy properties can be measured with reasonable computational time on future datasets from large-scale photometric surveys.

Finally, any new algorithm must be validated against known results from literature. Since we have developed {\sc mirkwood} to appeal to observers, we will use it to derive physical properties of galaxies from DR3 of the GAMA survey \citep{gama_driver2009}. In a recent work, \cite{bellstedt2020galaxy} formulated a novel SFH prior, and derived SFH and metallicty posteriors of $\sim 7000$ galaxies in the nearby universe. They were able to recreate the cosmic star formation rate density much better than using other parametric formulations of the SFH. We plan on using this same dataset and comparing our results with the GAMA Team.






==> INTRODUCTION.tex <==
\section{Introduction}\label{sec:introduction}

%One of the most powerful methods for deriving physical properties of galaxies involves the modeling of their Spectral Energy Distributions (SEDs). 
\subsection{Traditional SED Fitting}

Spectral energy distributions (SEDs) of galaxies are crucial in informing our understanding of the most fundamental physical properties, such as their redshifts, stellar population masses, ages, and dust content. %Different physical processes leave their imprint in different parts of the spectrum; the wider and more finely sampled the wavelength coverage, the more robust the interpretation of the various features of the SED is in terms of galaxy properties.
The task of extracting these properties by fitting models of the stellar photometry and dust attenuation to observations of galaxies is commonly known as SED fitting, and is one of the most common ways of deriving physical properties of galaxies. %\red{\sout{In brief, it is the process of iteratively comparing computer generated models of galaxy flux distributions (either in the form of photometry or spectroscopy) to their observed SEDs, and deriving the properties of the real data by minimizing the difference between them and the models.}}
In SED fitting, stellar populations are evolved with stellar population synthesis (SPS) models over an assumed star formation history (SFH), with an assumed stellar initial mass function (IMF) and through an assumed dust attenuation curve, to produce a composite spectrum. This resulting spectrum is then compared to the galaxy photometric observation under consideration, and the input assumptions are varied until there is a reasonable match between the two. The best fit model is then used to infer the physical properties of the concerned galaxy (see recent reviews by \citealt{walcher2011fitting, conroy2013modeling}). 

This technique has been transformational in turning observed data into inferred galaxy physical properties. %The success and reliability of this method depends on the quality of the available template spectra, and the robustness of the fitting algorithm. %While it would be impossible to summarize all the papers that have used SED modeling techniques in conjunction with HST-enabled observations of galaxies, it is indeed noteworthy frankly amazing how many aspects of galaxy evolution the combination of SED fitting and HST observations have touched. 
For instance, we now understand the evolution of the galaxy stellar mass function through z $\sim 7$ \citep{tomczak2014galaxy, grazian2015galaxy, leja2019a}, %(e.g. Tomczak et al., 2014; Gonzalez et al., 2011; Finkelstein et al., 2010; Grazian et al., 2015; Leja et al., 2019a), 
the diversity in shapes of galaxy SFHs \citep{papovich2011rising, leja2019b}, the nature of the star formation rate--stellar mass (SFR-M$^{\star}$) relation through z = 2 \citep{mobasher2008relation, iyer2018sfr}, the process of inside-out quenching \citep{jung2017evidence}, and the general shapes of galaxy dust attenuation curves at high-z \citep{salmon2016breaking}, all thanks to a combination of high quality data with SED fitting techniques. These developments have spurred -- and in turn have been accelerated by -- the development of modern SED fitting codes such as {\rm CIGALE} \citep{boquien2019cigale}, {\sc Prospector} \citep{leja_deriving_2017}, {\rm FAST} \citep{kriekfast2009}, and {\rm MAGPHYS} \citep{da2008simplemagphys}. These codes rely on Bayesian optimization and Markov Chain Monte Carlo (MCMC) sampling methods to explore the large input base of computer simulated SED templates for close matches with an observed SED, and consequently output its physical properties.% \citep{leja_deriving_2017}.

At the same time, this traditional method of fitting SEDs has been known to introduce potential uncertainties and biases in the derived physical properties of galaxies. At the core of the issue are assumptions regarding the model stellar isochrones, spectral libraries, the IMF, the SFH, and the dust attenuation law. Each of these choices can dramatically impact the derived physical properties. %As a telling example, let us examine in some detail the impact of the model galaxy star formation history used in SED fitting techniques.
%Another common issue is the difficulty of constraining the SFHs of galaxies.
%\textbf{modify the next line \red{please. i can't undersatand it!}}Similarly, the spectral signatures of multiple non-coeval generations of stars are can be degenerate with other physical effects such as varying stellar metallicity, and older stellar populations with high mass-to-light ratios are easily hidden in observed spectra, an effect sometimes referred to as `outshining' \citep{maraston2010star}. 
For example, \cite{acquaviva2015simultaneous} evaluated the effects that different modelling assumptions have on the recovered SED parameters, and found that the incorrect parameterizations of the star formation history can significantly impact the derived physical properties.   %\textbf{modify next two lines.}
This finding has been confirmed by the works of \citet{wuyts2009color, michalowski2014spatially, sobral2014stellar} and \citet{simha2014parametrising}, who have all found significant impact of SFH on the derived galaxy stellar mass in various observational datasets.  Similarly, \cite{iyer2017reconstruction} and \cite{lower_stellar_mass} found that fitting the SFH using simple functional forms leads to a bias of up to 70\% in the recovered total stellar mass. In addition, \cite{carnall2019vandels} demonstrated that such simple functional forms for SFH also impose strong priors on other physical parameters, which in turn bias our inference for fundamental cosmic relations, such as the stellar mass function (SMF) and the cosmic star formation rate density (CSFRD, \cite{ciesla2017sfr, leja_how_2019}), critical for answering crucial questions in the study of galaxy formation and evolution. Even with more complex SFH functions which have been able to better reproduce the CSFRD \citep{gladders2013imacs_lognormal}, individual stellar age estimates have been biased \citep{carnall2019vandels, leja2019a}. In a similar vein to SFH modeling, in their recent review \cite{salim2020dust} found that incorrect assumptions of the dust attenuation law, even within the commonly accepted family of locally-calibrated curves, can drive major uncertainties in the derived galaxy star formation rates.

To overcome some of these limitations of traditional SED fitting, two broad approaches have been introduced. The first has been to modify the SFH prior employed during SED fitting. This has been accomplished by either creating new functional, parametric forms for the SFH that result in lower biases in derived posteriors in physical parameters, for instance by being less subject to the `outshining bias' \citep{behroozi2013average, simha2014parametrising}, or by developing parameter-free (\emph{non-parametric}) descriptions of the SFH \citep{tojeiro2007, iyer2017reconstruction, iyer2019nonparametric, leja_how_2019}. The latter are those that allow for a number of flexible bins of star formation to vary in the SED modeling procedure in order to model the more complex star formation histories that likely represent real galaxies \citep{iyer2018sfr, leja2019new}. In \cite{lower_stellar_mass}, the authors used a subset of the hydrodynamical simulations used in this work, to study the biases introduced by various commonly used parametric forms of SFH on the derived stellar masses, and found that some of the most commonly used formulations -- `constant', `delayed-$\tau$' and `delayed-$\tau$ + burst' -- dramatically under-predict the true stellar mass. They then compared the performance against that obtained by using a non-parametric SFH model \citep{leja_deriving_2017}, and found significantly better results. Even so, there were a large number of catastrophic outliers, with errors of up to 40\% (see Figure 3 in their work). This is because SED fitting is inherently a complex task involving several moving parts, and SFH is only one of several model assumptions that go in it. As already mentioned, the assumed dust attenuation law is another factor that can significantly impact the derived galaxy properties (see Figure 2 in \citealt{salim2020dust}).% In their recent review, \cite{salim2020dust} demonstrated this by fitting SEDs from a cosmological simulation (akin to the analysis performed here), and while holding all other variables constant, compared the derived stellar masses assuming a \cite{calzetti1994dust} attenuation curve, and a standard SMC extinction \citep{pei1992interstellar_smc}. As is clear from Figure 2 in their work, uncertainty in dust attenuation law models can significantly impact derived physical properties from galaxies in traditional SED fitting techniques.

The upshot is that the uncertainties in the galaxy star formation history and star-dust geometry (as manifested in their dust attenuation curves) translate to significant uncertainties in the derived properties from traditional SED fitting techniques \citep{lower_stellar_mass, leja_deriving_2017, leja_how_2019, salim2020dust}. An alternative to SED fitting is to instead derive a mapping between the photometry of a galaxy and the underlying physical properties.   In this regard, machine learning techniques can serve as a potential alternative to traditional SED fitting.  In this paper, we demonstrate that machine learning is not only a suitable alternative, but potentially more accurate one.


%we give a brief introduction about supervised ML techniques and describe the algorithms that we propose to use. In Section 2, we describe our optimization process, which consists of comparing and selecting different estimators, as well as of data cleaning and feature selection and engineering. In Section 3, we apply the optimized algorithm to two sample data sets withi the SDSS catalogue, measuring the metallicity of SDSS galaxies and its uncertainty, and we compare our results to the current literature. In Section 4, we combine photometric data with spectroscopic measurements of emission lines fluxes and investigate the improvement in the determination of metallicity awarded by each one of them. In Section 5, we consider the applicability of our method to smaller samples, and we forecast the improvement in the metallicity measurement for the LSST main survey. 

%In Section 2 we describe the method in detail, including an overview of the machine learning techniques (2.1), the simulations used (2.2) and our method for generating synthetic spectra with spectacle, a stand-alone python module for generating spectra from cosmological simulations (2.3).1 Our results when trained and tested on the simulations are presented in Section 3. Section 4 details our modelling of the uncertainty contribution from the observational and modelling sources. We then apply our trained models to SDSS observations: Section 5.1 details the selection of our observational sample, Section 5.2 describes the VESPA SFH catalogue, and Section 5.3 presents our predictions. Finally, in Section 6 we discuss our results and avenues for future research, then summarise our conclusions in Section 7. We make all of our code for downloading the simulation and observational data, as well as training the CNNs, available online in the form of Jupyter notebooks.2 


==> METHODS.tex <==
\section{Proposed Method}\label{sec:methods_proposed_method}

%\input{METHODS_shapley_values}
%\input{METHODS_local_sols_global_probs}
%\input{intro_to_ml}
\input{proposed_method}
\input{uncertainty_quantification}
%\input{calibration}
\input{performance_metrics}

==> METHODS_local_sols_global_probs.tex <==
\section{Local Solutions to Global Problems}
Shapley values applied to feature imporance, as described in \S\ref{sec:shapley_values}, are defined as the sequential impact on the model's output of observing each input feature's value, averaged over all possible feature orderings. This means for each of all possible orderings, we introduce features one at a time into a conditional expectation of the model's output, then attribute the change in expectation to the feature that was introduced. In theory, however, Shapley values can be computed using any set function, not just conditional expectations. In this work, we use the SHapley Additive exPlanation (SHAP) python package \cite{shap1} (and associated SHAP values), and note that we are using conditional expectations to measure the impact of a set of features on the model.

Specifically, we use a local feature attribution method from the SHAP package called TreeExplainer, which is optimized for use with tree-based machine learning models \citep{shap2}. TreeExplainer bridges theory to practice by reducing the complexity of exact Shapley value computation from exponential to polynomial time. Using TreeExplainer allows us to combine \emph{local explanations}--feature importance for each sample/observation--to provide global insight into a model's behavior. This allows us to retain local faithfulness to the model while still capturing global patterns, resulting in richer, more accurate representations of the model's behavior. Each application presented below illustrates how local explanations can be used as building blocks for explainable machine learning. For all experiments we use an ensemble of five NGBoost models \citep{ngboost} since they natively output both the mean and the uncertainty of a prediction (in addition to supporting fast, exact, local explanations through TreeExplainer).

\input{shap_summary_plots}
%\input{shap_dependence_plot}
%\input{shap_decision_plots}
%\input{interaction_effects}
%\input{shap_clustering}
\input{metrics_for_prob_preds}


==> METHODS_preliminaries.tex <==
\section{Methodology: {\sc mirkwood} Algorithms}
\input{intro_to_ml}
\input{proposed_method}
\input{uncertainty_quantification}
\input{calibration}
\input{performance_metrics}

==> METHODS_shapley_values.tex <==
\section{Shapley Values}\label{sec:shapley_values}
Consider a dataset $\textbf{X}$ with $N$ features and $S$ samples $\textbf{X}=\left\{X^{(1)}_{1:S}, \ldots, X^{(N)}_{1:S}\right\},$ and a continuous, real-valued target variable vector $Y_{1:S}$. Given an instance (observation) $x \in \textbf{X} \in \textsc{R}^{1:N},$ a model $v$ forecasts the target as $v(x)$. In addition to this forecasting, we would also like to know if we can attribute the departure of the prediction $v(x)$ from the average value of the target variable $\bar{y} = \bar{Y}_{1:S}$ to each of the features (predictor variables) in the observed instance $x$? In a linear model, the answer is trivial :$v(x)-\bar{y}=\beta_{1} x^{(1)}+\cdots+\beta_{N} x^{(N)}$ (see Fig ()) [\textbf{INSERT CITATION FOR DE PRADO}]. We would like to do a similar local decomposition for any (non-linear) ML model.\footnote{As explained in \S\ref{sec:introduction} and evident from Figure {}, non-linear models provide much better predictions than linear ones.} Shapley values answer this \emph{attribution} problem through game theory \citep{shapley}. Specifically, they originated with the purpose of resolving the following scenario--a group of differently skilled participants are all \emph{cooperating} with each other for a collective reward; how should this reward be \emph{fairly} divided amongst the group? In the context of machine learning, the participants are the features of our input dataset $\textbf{X}$ and the collective \emph{payout} is the \emph{excess} model prediction (i.e., $v(x) - \bar{y}$). Here, we use Shapley values to calculate how much each individual feature \emph{marginally} contributes to the model output--both for the dataset as a whole (\emph{global explainability}) and for each instance (\emph{local explainability}).

While a goal of this paper is to explain the contributions of narrow- and broad-bands to various galaxy properties, for the sake of simplicity we chose to explain Shapley values using a toy example. Let us say that we operate a small hedge fund, and our team consists of three people: \emph{\underline{A}lice}, \emph{\underline{B}ob}, and\emph{\underline{C}arol}. On average, they manage to make approximately \$100,000 everyday ($\bar{y} = 100$ (thousand)). At the end of the year, we would like to distribute bonuses to our team members in direct proportion to their contribution to beating the average daily profit. Let us consider one day in particular, when owing partly to market volatility and partly to luck, today they make \$120,000 (i.e., excess income = 20 (thousand) dollars). Below, we delineate the process of determining each person's fair contribution to this number.

\begin{enumerate}
    \item First, we consider the $2^{N=3}$ possible coalitions (interactions) between the players (features), where some players may not participate (i.e., remain at their average value), and other may participate (depart from their average value). See Table \ref{table:coalitions}.
    \item Second, we use the coalitions table to compute the marginal contribution of each player conditional on the contribution of every other player. The marginal impact of changing \emph{A} after changing \emph{B} may differ from the marginal impact of changing \emph{B} after changing \emph{A}. Accordingly, we must account for all possible $N! = 6$ sequences of conditional effects. See Table \ref{table:marginal_conditional_contribution}.
    \item Finally, the \emph{Shapley value} of a player is calculated as the average conditional marginal contribution of that player across all the possible $N!$ ways of conditioning the predictive model $v$. See last row of Table \ref{table:marginal_conditional_contribution} and Equation \ref{eq:shapley_main}.
\end{enumerate}

\begin{table}%[h!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline $\text{Alice} \neq \overline{\text{Alice}}$ & $\text{Bob} \neq \overline{\text{Bob}}$ & $\text{Carol} \neq \overline{\text{Carol}}$ & $v(...) \left(= v[x \mid \ldots]\right)-\bar{y}$ \\
\hline 0 & 0 & 0 & $v(\varnothing) (= v[x \mid 000])-\bar{y} = 0$ \\
\hline 0 & 0 & 1 & $v(C) (= v[x \mid 001])-\bar{y} = 10$ \\
\hline 0 & 1 & 0 & $v(B) (= v[x \mid 010])-\bar{y} = 5$ \\
\hline 0 & 1 & 1 & $v(B,C) (= v[x \mid 011])-\bar{y} = 7$ \\
\hline 1 & 0 & 0 & $v(A) (= v[x \mid 100])-\bar{y} = 2$ \\
\hline 1 & 0 & 1 & $v(A,C) (= v[x \mid 101])-\bar{y} = 8$ \\
\hline 1 & 1 & 0 & $v(A,B) (= v[x \mid 110])-\bar{y} = 10$ \\
\hline 1 & 1 & 1 & $v(A,B,C) (= v[x \mid 111])-\bar{y} = \textcolor{orange}{20}$ \\
\hline
\end{tabular}
\caption{In a model with 3 features, there are $2^{3}=8$ possible interactions. For each interaction, we compute the departure of the model's forecast from its baseline (average value). We encode as `1' a feature that is not at its average value (it forms part of a \emph{coalition}), and `0' a feature that is at its average value. Thus $v(A,B)=v(B,A)$, $v(B,C)=v(C,A)$, $v(A,C)=v(C,A)$, and $v(A,B,C)=v(B,A,C)=v(A,C,B)$.}
\label{table:coalitions}
\end{table}

\iffalse
%similar plot to the one in /home/sgilda/Downloads/SSRN-id3637020.pdf, page 9
An attribution of the departure of a model's prediction, $f[x],$ from its average value, $\bar{y}$ Because addition is commutative, the sequence of the effects does not alter the result. Hence,
in a linear model, the attribution is invariant to the sequence of effects.
\fi

%\subsection{Coalitional Game Theory}

\begin{table}%[h!]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline Combination & \multicolumn{1}{|c|} {Alice} & \multicolumn{1}{|c|} {Bob} & \multicolumn{1}{|c|} {Carol} & Total \\
\hline $\mathrm{A}, \mathrm{B}, \mathrm{C}$ & $v(\mathrm{A})-v(\varnothing) = 2$ & $v(\mathrm{A}, \mathrm{B})-v(\mathrm{A}) = 8$ & $v(\mathrm{A}, \mathrm{B}, \mathrm{C})-v(\mathrm{A}, \mathrm{B}) = 10$ & \textcolor{orange}{20}\\
\hline $\mathrm{A}, \mathrm{C}, \mathrm{B}$ & $v(\mathrm{A})-v(\varnothing) = 2$ & $v(\mathrm{A}, \mathrm{C}, \mathrm{B})-v(\mathrm{A}, \mathrm{C}) = 12$ & $v(\mathrm{A}, \mathrm{C})-v(\mathrm{A}) = 6$ & \textcolor{orange}{20} \\
\hline $\mathrm{B}, \mathrm{A}, \mathrm{C}$ & $v(\mathrm{B}, \mathrm{A})-v(\mathrm{B}) = 5$ & $v(\mathrm{B})-v(\varnothing) = 5$ & $v(\mathrm{B}, \mathrm{A}, \mathrm{C})-v(\mathrm{B}, \mathrm{A}) = 10$ & \textcolor{orange}{20} \\
\hline $\mathrm{B}, \mathrm{C}, \mathrm{A}$ & $v(\mathrm{B}, \mathrm{C}, \mathrm{A})-v(\mathrm{B}, \mathrm{C}) = 13$ & $v(\mathrm{B})-v(\varnothing) = 5$ & $v(\mathrm{B}, \mathrm{C})-v(\mathrm{B}) = 2$ & \textcolor{orange}{20} \\
\hline $\mathrm{C}, \mathrm{A}, \mathrm{B}$ & $v(\mathrm{C}, \mathrm{A})-v(\mathrm{B}) = 3$ & $v(\mathrm{C}, \mathrm{A}, \mathrm{B})-v(\mathrm{C}, \mathrm{A}) = 12$ & $v(\mathrm{C})-v(\varnothing) = 10$ & \textcolor{orange}{20} \\
\hline $\mathrm{C}, \mathrm{B}, \mathrm{A}$ & $v(\mathrm{C}, \mathrm{B}, \mathrm{A})-v(\mathrm{C}, \mathrm{B}) = 13$ & $v(\mathrm{C}, \mathrm{B})-v(\mathrm{C}) = -3$ & $v(\mathrm{C})-v(\varnothing) = 10$ & \textcolor{orange}{20} \\
\hline Average & $6.3$ & $6.5$ & $8$ & \textcolor{orange}{20} \\
\hline
\end{tabular}
\caption{In a model with 3 features, there are $3! = 6$ possible sequences. We can use the interactions table to derive the marginal contribution of each feature in each sequence. The Shapley values are the averages per column.}
\label{table:marginal_conditional_contribution}
\end{table}

\iffalse
\begin{tabular}{l|l|l|l}
\multicolumn{1}{c|} { Sequence } & \multicolumn{1}{c|} {$x^{(1)}$} & \multicolumn{1}{c} {$x^{(2)}$} & \multicolumn{1}{c} {$x^{(3)}$} \\
\hline$x^{(1)}, x^{(2)}, x^{(3)}$ & $f[x \mid 100]$ & $f[x \mid 110]$ & $f[x \mid 111]$ \\
& $-f[x \mid 000]$ & $-f[x \mid 100]$ & $-f[x \mid 110]$ \\
\hline$x^{(1)}, x^{(3)}, x^{(2)}$ & $f[x \mid 100]$ & $f[x \mid 111]$ & $f[x \mid 101]$ \\
& $-f[x \mid 000]$ & $-f[x \mid 101]$ & $-f[x \mid 100]$ \\
\hline$x^{(2)}, x^{(1)}, x^{(3)}$ & $f[x \mid 110]$ & $f[x \mid 010]$ & $f[x \mid 111]$ \\
& $-f[x \mid 010]$ & $-f[x \mid 000]$ & $-f[x \mid 110]$ \\
\hline$x^{(2)}, x^{(3)}, x^{(1)}$ & $f[x \mid 111]$ & $f[x \mid 010]$ & $f[x \mid 011]$ \\
& $-f[x \mid 011]$ & $-f[x \mid 000]$ & $-f[x \mid 010]$ \\
\hline$x^{(3)}, x^{(1)}, x^{(2)}$ & $f[x \mid 101]$ & $f[x \mid 111]$ & $f[x \mid 001]$ \\
& $-f[x \mid 001]$ & $-f[x \mid 101]$ & $-f[x \mid 000]$ \\
\hline$x^{(3)}, x^{(2)}, x^{(1)}$ & $f[x \mid 111]$ & $f[x \mid 011]$ & $f[x \mid 001]$ \\
& $-f[x \mid 011]$ & $-f[x \mid 001]$ & $-f[x \mid 000]$
\end{tabular}
\fi
%that slide on Interaction Effects. Page 15

\textbf{\underline{Eliminating Redundancy}}: As we can appreciate from the numerical exercise in Tables \ref{table:coalitions} and \ref{table:marginal_conditional_contribution}, some calculations are redundant. For example, the marginal contribution of \emph{C} on sequence \emph{(A, B, C)} must be the same as the marginal contribution of \emph{C} on sequence \emph{(B, A, C)}, because (a) in both cases \emph{C} comes in third position, and (b) the permutations of \emph{(A, B)} do not alter that marginal contribution. The Shapley value of a feature $i$ can be derived as the average contribution of $i$ across all possible coalitions $S$, where $S$ does not include feature $i$:

\begin{align}\label{eq:shapley_main}
    \phi_{i}(v)=\sum_{S \subseteq N \backslash\{i\}} \frac{|S| !(|N|-|S|-1) !}{|N| !}(v(S \cup\{i\})-v(S))
\end{align}

The above equation describes a \emph{coalitional game} (the scenario described previously) with a set \textbf{N} of $|\textbf{N}|$ players. The function $v$ gives the value (payout) for any subset of those players. For example, if $S$ be a subset of \textbf{N}, then \emph{v(S)} gives us the value of that subset. Thus for a coalitional game (\textbf{N}, \emph{v}) Equation \ref{eq:shapley_main} outputs the value for feature \emph{i}, i.e. its the Shapley value.\footnote{Equation \ref{eq:shapley_main} computes the exact Shapley values by grouping the marginal conditional contributions in terms of coalitions $(S)$. For large $N,$ \cite{shap1} and \cite{shap2} have developed fast algorithms for the estimation of $\phi_{i}$} For ease of explanation, we focus our attention on calculating how many of the excess $20$ (thousand) dollars can be attributed to \emph{C}(arol), i.e. calculating the Shapley value for \emph{C}. We then examine the various components of Equation \ref{eq:shapley_main} and study their significance.
\begin{itemize}
    \item If we relate this back to the parameters of the Shapley value formula we have \textbf{N}$ = \{A, B, C\}$ and $i = C$. The highlighted section in Equation \ref{eq:shapley_highlight_0} (derived from Equation \ref{eq:shapley_main} by re-arranging some terms) says that we need to take our group of people and exclude the person that we are focusing on now. Then, we need to consider all of the possible subsets that can be formed. So if we exclude \emph{C} from the group we are left with \emph{{A, B}}. From this remaining group we can form the following subsets (i.e. these are the sets that \emph{S} can take on): $\varnothing, A, B, AB$. In total, we can construct four unique subsets from the remaining team members, including the null set.
    \begin{align}\label{eq:shapley_highlight_0}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{\textcolor{orange}{S \subseteq N \backslash\{i\}}}\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}(v(S \cup\{i\})-v(S))
    \end{align}
    \item Next, we focus on the highlighted term  in Equation \ref{eq:shapley_highlight_1}.
    \begin{align}\label{eq:shapley_highlight_1}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{S \subseteq N \backslash\{i\}}\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}\textcolor{orange}{(v(S \cup\{i\})-v(S))}
    \end{align}
    This refers to the \emph{marginal value} of adding player $i$ to the game. Specifically, we want to see the difference in the money earned daily if we add $C$ to each of our four subsets. We denote these four marginal values as: $\Delta v_{C, \varnothing}, \Delta v_{AC, A}, \Delta v_{BC, B}, \Delta v_{A B C, A B}$. Each of these as a different scenario that we need to observe in order to fairly assess how much \emph{C} contributes to the overall profit. This means that we need to observe how much excess money is produced if everyone is working at their average levels (i.e. the empty set $\varnothing$) and compare it to what happens if we only have \emph{C} working at above or below-average productivity. We also need to observe how much profit is earned by \emph{A} and \emph{B} working simultaneously and compare that to the profit earned by \emph{A} and \emph{B} together with \emph{C}, and so on.
    \item Next, the summation in the Shapley value equation is telling us that we need to add all them together. However, we also need to scale each marginal value before we do that, which we are provided this prescription by the highlighted part in Equation \ref{eq:shapley_highlight_2}.
    \begin{align}\label{eq:shapley_highlight_2}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{S \subseteq N \backslash\{i\}}\textcolor{orange}{\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}}(v(S \cup\{i\})-v(S))
    \end{align}
    It calculates how many permutations of each subset \emph{size} we can have when constructing it out of all remaining team members excluding feature (player) \emph{i}. In other words, given \textbf{$\lvert$N$\rvert$-1} features (players), how many groups of size \textbf{$\lvert$S$\rvert$} can one form with them? We then use this number to divide the marginal contribution of feature (player) $i$ to all groups of size \textbf{$\lvert$S$\rvert$}. For our scenario, we have that \textbf{$\lvert$N$\rvert$-1 = 2}, i.e. these are the remaining team members when we are left with when calculating the Shapley value for \emph{C}. In our case we will use that part of the equation to calculate how many groups we can form of size 0, 1, and 2, since those are only group sizes we can construct with the remaining players. So, for example, if we have that \textbf{$\lvert$S$\rvert$ = 1} then we get that we can construct 2 different groups of this size: \emph{A} and \emph{B}. This means that we should apply the following scaling factors to each of our 4 marginal values: $1\Delta v_{C, \varnothing}, \frac{1}{2}\Delta v_{A C, A}, \frac{1}{2}\Delta v_{B C, B}, 1\Delta v_{A B C, A B}$. By adding this scaling factor we are \emph{averaging out} the effect that the rest of the team members have for each subset size. This means that we are able to capture the \emph{average} marginal contribution of \emph{C} when added to a team of size 0, 1, and 2 \emph{regardless} of the composition of these teams.
    \item Next, we focus on the remaining term, highlighted in Equation \ref{eq:shapley_highlight_3}.
    \begin{align}\label{eq:shapley_highlight_3}
    \phi_{i}(v)=\textcolor{orange}{\frac{1}{|N|}} \sum_{S \subseteq N \backslash\{i\}}\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}(v(S \cup\{i\})-v(S))
    \end{align}
    So far we have averaged out the effects of the other team members for each subset size, allowing us to express how much \emph{C} contributes to groups of size 0, 1, and 2. The final piece of the puzzle is to \emph{average out} the effect of the group size as well, i.e. how much does \emph{C} contribute \emph{regardless} of the size of the team (number of explanatory features in the data set). For our scenario we do this by dividing with 3 since that is the number of different group sizes that we can consider. With this final step, we arrive at the point where can finally compute the Shapley value for \emph{C}. We have observed how much she marginally contributes to all different coalitions the team that can be formed. We have also averaged out the effects of both team member composition as well as team size which finally allows us to compute the Shapley value for \emph{C}:
    \begin{align}\label{eq:shapley_final}
        \phi_{C}(v) &= \frac{1}{3} \sum\left(1\Delta v_{C, \varnothing}, \frac{1}{2} \Delta v_{A C, A}, \frac{1}{2} \Delta v_{B C, B}, 1\Delta v_{ABC, AB}\right) \nonumber \\
        &= \frac{1}{3} \sum\left(1\times 10, \frac{1}{2} \times 6, \frac{1}{2} \times 2, 1\times 10\right) \nonumber \\
        &= 8
    \end{align}
    Comparing Equation \ref{eq:shapley_final} with the Shapley value for \emph{C} in the last row of Table \ref{table:marginal_conditional_contribution}, we see that they match exactly.
\end{itemize}

After calculating the Shapley values for the rest of the players, we can then determine their individual contributions to the excess 20 (thousand) dollars earned today, allowing us to fairly divide the bonus amongst all team members:
\begin{align}
    20 &=v(\{A, B, C\}) \nonumber \\
    &=\phi_{A}(v)+\phi_{B}(v)+\phi_{C}(v)
\end{align}
This is also evident from the last row of Table \ref{table:marginal_conditional_contribution}, where the Shapley values for \emph{A}, \emph{B}, and \emph{C} add to the total of 20.


\textbf{\underline{Properties}}:
As they apply to local explanations of predictions from machine learning models, Shapley values have some nice uniqueness guarantees \citep{shapley}. As described above, Shapley values are computed by introducing each feature, one at at time, into a conditional
expectation function of the model's output, $v_{x}(S) \approx E[v(x) | x_{S}]$, and attributing the change produced at each step to the feature that was introduced; then averaging this process over all possible feature orderings. Shapley values are provably the only possible method in the broad class of \emph{additive feature attribution methods} \cite{shap1} that simultaneously satisfy four important properties of \emph{fair} credit-attribution: \emph{efficiency}, \emph{symmetry}, \emph{missingness}, and \emph{additivity}.
\begin{enumerate}
    \item \emph{Efficiency/ Local Accuracy}: The sum of the Shapley values of all features (players) equals the value of the total coalition. That is, the value of $20$ in the bottom-rightmost corner in Table \ref{table:coalitions} is the same as the $20$ in the bottom-rightmost cell in Table \ref{table:marginal_conditional_contribution}.
    \item \emph{Missingness}: If a feature (player) never adds any marginal value regardless of the coalition, its payoff (Shapley value $\phi_{i}(v)$) is 0. That is, if: $v(S \cup \{i\}) = v(S) \forall $ subsets of features \emph{S}, then $\phi_{i}(f) = 0$.
    \item \emph{Symmetry}: All players have a fair chance to join the game. That’s why Table \ref{table:coalitions} lists all the permutations of the players. If two players always add the same marginal value to any subset to which they are added, their payoff portion should be the same. In other words, $\phi_{i} = \phi_{j}$ IIF feature \emph{i} and feature \emph{j} contribute equally to all possible coalitions.
    \item \emph{Additivity}: A function with combined outputs has as Shapley values the sum of the constituent ones. For any pair of games $v, w$, $\phi(v+w) = \phi(v)+\phi(w)$, where $(v+w)(S)=v(S)+w(S) \forall S$. This property allows us to combine Shapley values from $n$ different models, thus enabling interpretability for ensembles. 
\end{enumerate}

\iffalse
\textbf{\underline{Interaction Effects}}: An interaction effect occurs when the effect of one variable on the output depends on the value of another variable. The estimation of interaction effects requires having an accurate attribution of the individual effect of the variables involved. This makes Shapley values particularly useful for estimating these. For $i \neq j$:
\begin{align}
    \phi_{i, j}=\sum_{S \subseteq(X \backslash\{i, j\})} \frac{|S| !(|N|-|S|-2) !}{2(|N|-1) !} \delta_{i, j}(S), \nonumber \\
    \delta_{i, j}(S)=v(S \cup\{i, j\})-v(S \cup\{i\})-v(S \cup\{j\})+v(S)
\end{align}
\fi


\iffalse
%https://towardsdatascience.com/explain-your-model-with-the-shap-values-bc36aac4de3d
Lloyd Shapley came up with this solution concept for a cooperative game in 1953. Shapley wants to calculate the contribution of each player in a coalition game. Assume there are N players and S is a subset of the N players. Let v(S) be the total value of the S players. When player i join the S players, Player i’s marginal contribution is v(S union {i})- v(S). If we take the average of the contribution over the possible different permutations in which the coalition can be formed, we get the right contribution of player i:
\fi

\iffalse
\begin{align}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{S \subseteq N \backslash\{i\}}\left(\begin{array}{c}
|N|-1 \\
|S|
\end{array}\right)^{-1}(v(S \cup\{i\})-v(S))
\end{align}
\fi


This plot is made of all the dots in the train data. It demonstrates the following information:
Feature importance: Variables are ranked in descending order.
Impact: The horizontal location shows whether the effect of that value is associated with a higher or lower prediction.
Original value: Color shows whether that variable is high (in red) or low (in blue) for that observation.
Correlation: A high level of the `alcohol' content has a high and positive impact on the quality rating. The `high' comes from the red color, and the `positive' impact is shown on the X-axis. Similarly, we will say the `volatile acidity' is negatively correlated with the target variable.


==> RELATED_WORK.tex <==
\subsection{Machine Learning and SED Fitting}\label{sec:related_work}
To explore the complex and degenerate parameter space more efficiently, machine learning (ML) has emerged as an alternative tool for deriving the physical parameters of galaxies. Unlike traditional SED fitting procedures, including those utilizing novel non-parametric SFH priors, ML algorithms are able to directly learn the relationships between the input observations (either photometric of spectroscopic) and the galaxy properties of interest without the need for human-specified priors. With ML, the priors themselves become learnable. This is possible because ML algorithms learn from the entire population ensemble, learning not just the mapping between individual galaxy observations and physical properties, but also the distribution of properties.%Using a training data set consisting of samples (fluxes in different bands) with known output values (galaxy physical properties), they attempt to learn the underlying data-generating distribution (\emph{supervised learning}, Section \ref{sec:methods_intro_to_ml}).

 %(Sadeh et al. 2016; Ball et al. 2008; Hogan et al. 2015; Masters et al. 2015; more).
\cite{lovell2019learning}) trained convolutional neural networks (CNNs, \cite{krizhevsky2012imagenet_cnn}) to learn the relationship between synthetic galaxy spectra and high resolution SFHs from the \textsc{EAGLE} \citep{schaye_2015_eagle} and \textsc{Illustris} \citep{vogelsberger2014introducingillustris} simulations. \cite{stensbo2017sacrificing} estimated specific star formation rates (sSFRs) and redshifts using broad-band photometry from SDSS (Sloan Digital Sky Survey, \cite{sdss_eisenstein2011}). \cite{surana2020predicting} used CNNs with multiband flux measurements from the GAMA (Galaxy and Mass Assembly, \cite{gama_driver2009}) survey to predict galaxy stellar mass, star formation rate, and dust luminosity. \cite{simet2019comparison} used neural networks trained on semi-analytic catalogs tuned to the CANDELS (Cosmic Assembly Near-infrared Deep Extragalactic Legacy Survey, \cite{grogin2011candels}) survey  to predict stellar mass, metallicity, and average star formation rate. Owing to their superior ability in capturing non-linearity in data, ML-based models have seen applications in almost every field of astronomical study, including identification of supernovae \citep{disanto2016}, classification of galaxy images %\red{add citations to papers by chris conselice's group who has done a lot here, as well as some student of brant robertsons who has some nice code called morpheus about this. also this paper: https://arxiv.org/pdf/2004.11981.pdf -- best to read these papers and look in their intros for further referencing as we really want to get the referencing complete}
\citep{ml_morphology0,ml_morphology1, hausen2020morpheus,ciprijanovic2020deepmerge,barchi2020machine}, and categorization of signals observed in a radio SETI experiment \citep{harp2019}. With the exponential growth of astronomical datasets, ML based models are slowly becoming an integral part of all major data processing pipelines \citep{siemiginowska2019astro2020}. \cite{baron2019machine} provides a comprehensive and current overview of the application of machine learning methodologies to astronomical problems.

\subsection{This Paper}
In this paper we introduce \textsc{mirkwood}, a fully ML-based tool for deriving galaxy physical parameters from multi-band photometry, while robustly accounting for various sources of uncertainty.  We %discuss the potential for ML techniques in SED fitting, and
compare {\sc mirkwood}'s performance with that of the current state-of-the-art Bayesian SED fitting tool \textsc{Prospector}, by using data from galaxy formation simulations for which we have ground-truth values\footnote{While one could consider using observed photometric data of real galaxies instead, a glaring lack of well-defined ground truth physical parameters -- independent of any inference tool employed -- would make comparisons between results from \textsc{mirkwood} and any traditional SED fitting code difficult. %A tenable workaround could be to consider only those galaxies for which simultaneous spectroscopic data, and hence high-confidence physical parameters, are available. However, with the intention of keeping this work self-contained, we eschew this in favor of using multi-band SEDs from hydrodynamical simulations that have been empirically shown to closely, if not perfectly, match the properties of matter in the known universe, thus enabling a helpful `proof-of-concept' based purely on photometry.
}. To do this, we first create mock SEDs from three different cosmological hydrodynamical simulations (via the procedure discussed in detail in Section \ref{sec:data} and illustrated in Figure \ref{fig:pd_sed}) -- \textsc{Simba}, \textsc{EAGLE}, and \textsc{IllustrisTNG}. We then fit GALEX, HST, Spitzer, Herschel, and JWST photometry of these mock SEDs to extract stellar masses, dust masses, stellar metallicities, and instantaneous SFRs (defined as the mean SFR in the past 100 Myrs from the time of observation) using the publicly available SED fitting software {\sc Prospector} \citep{leja_deriving_2017} with the state-of-the-art non-parametric SFH model from \cite{leja_deriving_2017, leja2019a} (Section \ref{sec:data}). We repeat this exercise using \textsc{mirkwood}, and compare both sets of derived galaxy properties to their true values from simulations.

The rest of this paper is organized as follows. %In Section \ref{sec:related_work}, \green{Does it make sense to include the previous section in this outline?} we give a brief overview of non-traditional SED fitting methods that have been used over the past few years to derive different galaxy properties from both photometric and spectroscopic observations, focusing on their strengths and weaknesses.
In Section \ref{sec:data} we describe both our data and the traditional SED fitting technique in significant detail, including the three hydrodynamical simulations (Section \ref{sec:data_sims}), the method to select galaxies of interest from these simulations (Section \ref{sec:data_galaxyselection}), the dust radiative transfer process used to create SEDs (Section \ref{sec:data_radiativetransfer}), and finally the Bayesian code used to fit these SEDs to derive galaxy properties (Section \ref{sec:data_prospector}). In Section \ref{sec:methods_proposed_method} we describe in detail the SED modeling procedure using our proposed model \textsc{mirkwood}. We describe how \textsc{mirkwood} robustly estimates uncertainties in its predictions (uncertainty quantification, Section \ref{sec:methods_uncertainty}), %how we \emph{post hoc} correct overly optimistic predictions (probability calibration, Section \ref{sec:calibration}),
and introduce metrics to quantify performance gains with respect to traditional SED fitting (Section \ref{sec:methods_metrics}). In Section \ref{sec:results}, we investigate the improvement in the determination of the four galaxy properties. Finally, in Section \ref{sec:discussion} we summarize our findings, and suggest possible improvements to both the proposed model and to areas of application. Throughout we assume a Planck 2013 cosmology with the following parameters: $\Omega_m = 0.30$, $\Omega_\lambda = 0.70$, $\Omega_b = 0.048$, $h = 0.68$, $\sigma_8 = 0.82$, and $n_s = 0.97$. %We make all of our code for downloading the simulations as well as training \textsc{mirkwood}, available online in the form of python scripts\footnote{\url{abc.github.com}}.

%\red{I think these following paragraphs are redundant, and don't add any new information, and could/should be cut}\red{\sout{In this work, we develop for the first time an ML-based tool that is able to cover several deficiencies in the treatments listed above \red{wait what deficiencies? the last few paragraphs are all about how awesome ML is.}. \red{First \sout{For one}},  \red{(Though i'm still not sure what deficiencies we're beating, and how training on 3 separate simulations helps us do that)} we train on a combination of data from three separate simulations, and train our model in a way that is able to account for the inter-dependencies between galaxy properties. Any supervised ML algorithm is only as generalizable as its training set; by utilizing SEDs from three diverse state-of-the-art simulations with varying physical assumptions about the universe, we attempt to marginalize over each simulation's deviation from reality. \red{Second?} To the best of our knowledge, this is the first work to use ML to predict galaxy properties in a way that captures their intrinsic inter-relationships. For instance, \red{() and ()} both create different neural networks for predicting each of the different galaxy properties in their respective works, and thus lose out on valuable correlations between properties, such as the mass-metallicity relationship (). \textsc{mirkwood} is also the first tool to differentiate between systematic and statistical uncertainties, explain their relative significance vis-a-vis prediction of galaxy properties, and has the ability to inform the observer when a particular observation is too different from the samples in the training set and thus any results from \textsc{mirkwood} should be suspect, instead of confidently outputting incorrect and potentially catastrophic predictions. \textsc{mirkwood} is capable of handling missing observations, and of propagating observational uncertainties to galaxy properties. Finally, it is the first tool to use Shapley values to weigh input features in accordance with their contribution to the predictions, thus enabling the observer a peek into the inner machinations of the decision-making procedure of the model.}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
As we emphasize in Section \ref{sec:introduction}, one of the more dominant yet poorly constrained components of SED fitting is the assumed form of the star formation history (SFH). The most common models for SFHs are parameterized by a simple functional form, and the parameters varied in the SED fit describe that functional form. Hereafter, we refer to these as “parametric” star formation histories. Examples include the τ and delayed-τ models, which model the SFH as exponentially declining with some characteristic e-folding time. Although these models are computationally efficient and match the SFHs of galaxies in a closed box with constant star formation efficiency, the restricted nature of the functional forms does not match the diversity of true galaxy SFHs (Gallagher et al. 1984; Sandage 1986; Lee et al. 2009; Oemler et al. 2013; Simha et al. 2014; Diemer et al. 2017). The assumed SFH and associated priors can also strongly impact the inferred physical properties of galaxies (Simha et al. 2014; Iyer & Gawiser 2017; Salmon et al. 2015; Carnall et al. 2019). For instance, Curtis-Lake et al. (2020) found that the SFR-M∗ relation is sensitive to the priors used in the delayed-τ SFH employed in SED modeling. Michaowski et al. (2012) found that the assumed star formation history model had the largest impact out of all other SED model components on the stellar masses inferred for observations of sub-millimeter galaxies (SMGs). Similarly Dudzeviit et al. (2019) found that the average difference between the stellar masses predicted by the magphys SED model and the true stellar masses for galaxies from the eagle cosmological simulation was close to 0.5 dex. This bias, attributed to the assumed SFH module, is consistent with the earlier results of Michaowski et al. (2012).

Parametric SFHs with more complexity have also been explored in the literature (e.g. Pacifici et al. 2012; Simha et al. 2014; Ciesla et al. 2017). An example is a lognormal parametrization, which has been shown to reproduce the evolution of the cosmic star formation rate history (Gladders et al. 2013) and provide a reasonable match to the Illustris galaxy SFHs (Diemer et al. 2017). However, as shown in Carnall et al. (2019) and Leja et al. (2019a), the log-normal parameterization still suffers from similar stellar age biases as the simpler parametric forms. This happens because the SFH is constrained to either have recent star formation or have a population of old stars (Leja et al. 2019a) – a consequence of the rigid exponential functional form. Moreover, Diemer et al. (2017) fit a log-normal SFH directly to the SFHs of the Illustris galaxies instead of via SED modeling where all galaxy properties must be inferred simulatenously, thus biases such as outshining (Papovich et al. 2001) did not affect the fit. 

Recently, a series of models employing nonparametric forms for galaxy SFHs in SED modeling have been developed in an attempt to minimize the effect of these systematic biases. These nonparametric SFH models have been shown to have the flexibility to reasonably reproduce the variation in SFHs seen in observations and galaxy formation simulations. Some nonparametric SFHs are modeled as a function of families of SFHs that effectively cover the space of all physical SFHs, as developed in Iyer & Gawiser (2017) with the Dense Basis method and improved upon in Iyer et al. (2019) which employs Gaussian Processes rather than parametric SFH families. Other methods model the SFH of a galaxy as a piece-wise function with multiple bins of constant star formation rate. Examples of this type include moped (Reichardt et al. 2001); vespa (Tojeiro et al. 2007); and propsector (Johnson et al. 2019; Leja et al. 2017; Leja et al. 2019a); as well as the SFH models for the Carnegie-Spitzer-IMACS survey (Kelson 2014; Dressler et al. 2016); and grism as used in Morishita et al. (2019).

While the aforementioned authors explored the impact of nonparametric star formation histories on observational data sets, the method is yet to be groundtruthed against the true stellar mass of the galaxy. Previous studies, including Leja et al. (2019a), have focused on simple tests of efficacy such as understanding how both nonparametric and traditional parametric SFH models behave when SFH assumptions of the model are violated. Leja et al. (2019b) demonstrated that galaxies selected from the 3D-HST photometry catalog (Skelton et al. 2014) were inferred systematically more massive and older when modeled with nonparametric SFHs in prospector compared to previously published results using parametric SFHs. Comparisons between simulated galaxy properties and the results inferred using SED modeling have primarily been limited by simulation technique or sample size (e.g. Finlator et al. 2007; Hayward & Smith 2015). Iyer & Gawiser (2017) compared results using the Dense Basis method for galaxies from a semi-analytic model (SAM) and a hydrodynamic simulation and found reasonable agreement but did not compare results to SED fits using a simpler parametric model.


%https://arxiv.org/pdf/2002.03578.pdf
The two can be broadly divided into two themes -- using non-parametric formalisms of star formation history, and using machine learning models to replace traditional SED fitting entirely.

Deep learning networks generally perform very well in capturing the non linearity in data. Convolutional neural network (CNN), a special type of deep learning network, is now witnessing an explosion of applications in various fields of research, including astronomy. Within the last two years, CNNs have been successfully applied for the classification of galaxy and radio galaxy images in Barchi et al. (2019) and Lukic et al. (2018) respectively. CNNs have also been used in categorization of signals observed in a radio SETI experiment (Harp et al. 2019). Lovell et al. (2019) have also trained CNNs to learn the relationship between synthetic galaxy spectra and high resolution SFHs from the EAGLE (Schaye et al. 2015) and Illustris (Vogelsberger et al. 2014) simulations.

Deep learning has been successfully applied in astronomy to classification problems. Zhang & Zhao (2006) used Bayesian Belief Networks (BBN), Multilayer Perceptron (MLP) networks and Alternating Decision trees (ADtree) for separating quasars from stars. Abraham et al. (2012) have used a machine learning classifier trained on a subset of spectroscopically confirmed objects, classifying them into stars, galaxies and quasars. D’Isanto et al. (2016) provide a comparison of various machine learning methods for tasks such as identification of cataclysmic variables, separation between galactic and extragalactic objects and identification of supernovae. Brescia et al. (2015) used MLP with Quasi Newton Algorithm to characterize the physical nature of the large number of objects observed by modern multiband digital surveys. Similarly, deep learning has also been successfully used to build regression models. For example, Guill´en et al. (2019) have used deep neural networks for the estimation of the muon content of extensive air showers when measured on the ground. Pearson et al. (2019) have implemented deep learning CNNs for estimating strong gravitational lens mass model parameters.

From the diversity of applications mentioned above, it is clear that deep learning approaches have proven useful in tackling a number of astronomical problems. In this work, we attempt to reproduce the capabilities of stellar population synthesis (SPS) models (see Conroy (2013) for a comprehensive review) via a deep learning approach. SPS models combine our understanding of the properties of stars as traced by stellar evolution and star formation histories. The spectral energy distribution of a stellar population in a galaxy is modulated by the presence of dust which tends to absorb or scatter stellar photons at short wavelengths. SPS models are physically well motivated and encapsulate a vast and ever growing literature that provides us with ever more sophisticated models. The complexity and sophistication of such modeling comes at a price - finding the best model within the vast parameter space (consisting of millions of possible models) is a compute intensive process. A machine learning approach holds the promise of leaving the building of this complex non-linear model to a machine suitably trained with a large dataset of examples.

In this work, we train a deep learning model to predict what are perhaps the three most basic parameters that are used to characterise the star formation process in galaxies - the current star formation rate (SFR), dust luminosity (DL) and stellar mass (SM). SM is a rough proxy for the integrated star formation in a galaxy throughout its history while the dust luminosity is a measure of the amount of dust in the galaxy. The data we use are from the GAMA (Galaxy And Mass Assembly; Driver et al. (2011)) survey. At its core, GAMA is a spectroscopic survey of ∼300,000 galaxies down to r < 19.8 mag over ∼ 286 deg2, which was carried out using the AAOmega multi-object spectrograph on the AngloAustralian Telescope (AAT). The core spectroscopic survey has been greatly augmented by multiwavelength observations of the GAMA fields with a wide variety of telescopes. We use the GAMA survey Panchromatic Data Release (PDR) catalog (Driver et al. 2016) which includes fluxes in upto 21 broadband filters for 120,114 galaxies. For each galaxy the catalog includes position information (RA/Dec), 21 band flux values along with individual errors, a spectroscopic redshift and stellar mass, star formation rate and dust luminosity. The last three parameters are determined using a stellar population synthesis code viz. magphys. This is one of the most widely used SED fitting codes which has been successfully applied on galaxy samples spannig a wide range of galaxy stellar masses, star formation rates and morphological types (e.g., da Cunha et al. 2010; Berta et al. 2013; Viaene et al. 2014; Chang et al. 2015; Driver et al. 2016; Bait et al. 2017; Driver et al. 2018). Our deep learning models are thus limited by the weaknesses of magphys (for instance, the active galactic nuclei’s contribution to the SED is not modeled in this code). In regions of parameter space where magphys is a poor model of the underlying physical reality, our deep learning model will also be a poor representation of the physical reality. Keeping this caveat in mind, we will proceed with our modeling. For constructing our deep learning model, we used the 21 band data consisting of far ultra-violet (UV) and near UV (from GALEX), the five Sloan Digital Sky Survey bands: ugriz, near infrared bands: X, Y, J, H, K, WISE mid-infrared bands: W1, W2, W3, W4, and the five Herschel bands: P100, P160, S250, S350, S500.

The spectroscopic redshift listed in the PDR catalog is used as an additional input parameter for our model. In Section 2, we introduce the deep learning algorithm and the data preprocessing we have carried out. In Section 3, we describe and discuss our results and we conclude in Section 4.


%%%https://arxiv.org/pdf/1905.08996.pdf



The ML techniques are only applicable within the limits of the training data. Any extrapolation of them to a different redshift or mass regime would lead to errors in the final estimate. However, a distinct advantage of ML is that one could incorporate extra information (i.e. morphology, galaxy light profile) within the algorithm. The ML techniques are divided into two categories: supervised and unsupervised. In supervised ML, the input attributes (magnitudes and colors) are provided along with the output (redshift) and directly used for training in the learning process (Lima et al. 2008; Freeman et al. 2009; Gerdes et al. 2010). Here, the learning process is supervised by the input parameters. The unsupervised techniques do not use the desired output values (e.g. spectroscopic redshifts) during the training with only the input attributes used. Due to its limitations, this is not frequently used.


We expect that this method will carry systematic uncertainties that are independent of those from SED fitting, so that our results will complement and strengthen the results of these approaches. Another strength of a machine learning-based approach is that the algorithm learns from the population ensemble, learning not only the correspondence between individual spectra and star formation histories, but also which star formation histories are common and which are unlikely, something that would be analogous in Bayesian parameter estimation to learning the SFH prior.

The use of ML methods has so far been limited mainly to measuring photometric redshifts of galaxies. This is because the ML algorithms can be more easily trained using the spectroscopic redshifts whereas for other parameters such true and unambiguous estimates are hard to obtain. Detailed comparisons have been performed between different methods and algorithms measuring photometric redshifts (Carrasco Kind & Brunner 2013; Dahlen et al. 2013) and masses (Mobasher et al. 2015) of galaxies. However, except in a few cases where ML techniques are used (MCC and neural net) these were mostly based on different variants of template fitting using observed or model SEDs. In particular, very few studies have performed a comparison of different ML techniques. A recent study has used Bayesian combination of photometric redshift Probability Density Functions (PDFs) using different ML methods to improve estimates of photometric redshifts (Carrasco Kind & Brunner 2014). However, no such study has been performed for other physical parameters of galaxies.

In this paper we use different ML techniques to measure the stellar mass and star formation rates of galaxies with available photometric data and photometric redshifts using a training set of semianalytic galaxies from (Lu et al. 2014). The test sample in this study is from the Hubble Space Telescope (HST) Cosmic Assembly Near-infrared Deep Legacy Survey (CANDELS) GOODS-South field. This has imaging data in optical (ACS) and near-infrared (WFC3) wavelengths as well as Spitzer Space Telescope mid-infrared (IRAC) bands. We describe the CANDELS data and semianalytic galaxies in section 2, give an overview of the neural network ML algorithm we use in section 3, test our neural networks with a semianalytic test set in section 4, and finally apply our networks to CANDELS data in section 5, with summary and conclusions in section 6. Throughout the paper, we assume the cosmology of the simulation used to generate the mock catalog and semianalytic galaxies: ΩM = 0.27, ΩΛ = 0.73, Ωb = 0.044, h = 0.7, n = 0.95, and σ8 = 0.82.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5https://arxiv.org/pdf/1903.10457.pdf


Here we propose an alternative approach, using supervised machine learning algorithms to ‘learn’ the relationship between the SFH and the SEDs of galaxies. In contrast with SED fitting, where the SFH is built from some ensemble of simple stellar populations to maximise the resemblance in SED space, machine learning directly learns the relationship between the spectra and the entire SFH. We expect that this method will carry systematic uncertainties that are independent of those from SED fitting, so that our results will complement and strengthen the results of these approaches. Another strength of a machine learning-based approach is that the algorithm learns from the population ensemble, learning not only the correspondence between individual spectra and star formation histories, but also which star formation histories are common and which are unlikely, something that would be analogous in Bayesian parameter estimation to learning the SFH prior.

A number of recent studies have explored the effect of priors on derived SFHs in SED fitting approaches. Carnall
et al. (2019) showed that parametric approaches implicitly
impose a strong prior on the SFH that can lead to unrealistically tight posterior constraints on the SFR, and Leja
et al. (2019) showed that even non-parametric fits are sensitive to the prior SFH distribution, particularly where the
data are poor. Pacifici et al. (2013) proposed using SFHs
from a semi-analytic model to generate a library of SEDs
to be used in an SED fitting algorithm, and found that
these simulation-motivated templates prefer symmetric or
rising SFHs at intermediate redshifts (0.2 < z < 1.4), compared to the exponentially declining forms predicted using
simple stellar populations. Finally, Wilkins et al. (2013a)
show that using simulation-motivated enrichment and starformation histories leads to more accurate stellar mass estimates from colour information only. These studies highlight
the importance of the explicitly or implicitly assumed prior
distribution of SFHs.

Machine learning methods are becoming an increasingly
popular tool for Astronomers (Ball & Brunner 2010; Baron
2019). This is particularly the case where there is abundant
low quality data for which expensive, higher quality data
can be obtained and used for supervised training. However,
a supervised machine learning algorithm is only as good as
its learning sample. The main challenges to applying these
techniques to measure properties such as star formation histories have been the following: assembling a sample of galaxies for which the “true” star formation history is known; and
making sure that properties of the ensemble (the distribution of properties and their relationship to one another) are
a fair snapshot of the real Universe. However, there has been
significant recent progress from multiple independent teams
on high-resolution cosmological models of galaxy evolution,
which has for the first time provided the potential to test
this technique (e.g. Simet et al. 2019).

Hydrodynamic cosmological simulations in particular are able to resolve stellar populations, producing realistic, high resolution SFHs by taking into account a number of effects, such as environmental interactions, mergers, and stellar and AGN feedback (Somerville & Dav´e 2015). EAGLE (Schaye et al. 2014) and Illustris (Genel et al. 2014) are two recent hydrodynamic simulations that reproduce a number of key galaxy distribution functions. Both are necessarily tuned to a small number of observational constraints due to their limited resolution, which requires subgrid models to model physical processes below the simulation scale. Despite this, a number of observables not included in the tuning are simultaneously reproduced. Of interest for this study are the distributions of colours and photometric magnitudes, which are well reproduced in both models (Trayford et al. 2015; Torrey et al. 2015). The recent convergence of such detailed models with the observations, and within sufficiently large simulated volumes, has finally enabled them to be used as training sets for machine learning models.
\fi


==> RESULTS.tex <==
\section{Results}\label{sec:results}

%%%% Chained vs Unchained Scatter
\begin{figure*}[!htbp]
\gridline{\leftfig{z_snr=5_20201108.pdf}{0.48\textwidth}{(a)}
          \rightfig{Calibration_z_snr=5_20201108.pdf}{0.48\textwidth}{(b)}
          }
\gridline{\leftfig{SHAPz0_z_snr=5_20201108.pdf}{0.48\textwidth}{(c)}
          \rightfig{SHAPz2_z_snr=5_20201108.pdf}{0.48\textwidth}{(d)}
          }
\gridline{\leftfig{Epis_z0_z_snr=5_20201108.pdf}{0.48\textwidth}{(e)}
          \rightfig{Epis_z2_z_snr=5_20201108.pdf}{0.48\textwidth}{(f)}
          }
\caption{{\bf Performance Characteristics of {\sc mirkwood} SED fitting: Galaxy redshifts.} %We demonstrate the significant improvements of {\sc mirkwood} over traditional SED fitting software by comparing the recovered vs true redshifts.
\textbf{(a,b)} \textbf{Validating predicted means and uncertainties, respectively.} %We plot the mean redshifts derived by {\sc mirkwood} against their ground truth values.
In \textbf{(a)} we see that given a test sample, our model is accurately able to predict the mean redshifts of z=0 and z=2 used in this work. The horizontal orange line in \textbf{(b)} indicates that the predicted errors from {\sc mirkwood} are extremely small/tight, and that our assumption of normal distribution of redshifts is incorrect. \textbf{(c,d)}: \textbf{SHAP summary plots for z=0 and z=2, respectively}. These show the relative importance of each feature in predicting the redshift. For instance, in \textbf{(c)}, flux at 1.49$\mu$m has a high and positive impact on the predicted redshift. \textbf{(e,f)} \textbf{Outlier detection, for z=0 and z=2 respectively.} Epistemic uncertainty (on the y-axis) is high when informative features are sparse in the training set. Here we do not see any trends for $\sigma_{e}$ since there are several equally important bands.% We believe this is due to the incorrect assumption of Gaussian distribution of redshifts, and in future work we will explore using Bernoulli distribution instead.  The `high' comes from the red color, and the `positive' impact is shown on the y-axis. Each of these convey several pieces of information -- (i) \emph{Impact:} the vertical extent for a feature above or below the y=0 line shows whether its effect is associated with a higher or lower prediction for redshift; \emph{Original value:} color shows whether the flux in a band is high (in red) or low (in blue); and \emph{Correlation:}
\label{fig:redshift}}
\end{figure*}


\begin{figure*}[!htbp]
\gridline{\leftfig{Mass_snr=5_20201108.pdf}{0.48\textwidth}{(a)}
          \rightfig{Calibration_Mass_snr=5_20201108.pdf}{0.48\textwidth}{(b)}
          }
\gridline{\leftfig{SHAPz0_Mass_snr=5_20201108.pdf}{0.48\textwidth}{(c)}
          \rightfig{SHAPz2_Mass_snr=5_20201108.pdf}{0.48\textwidth}{(d)}
          }
\gridline{\leftfig{Epis_z0_Mass_snr=5_20201108.pdf}{0.48\textwidth}{(e)}
          \rightfig{Epis_z2_Mass_snr=5_20201108.pdf}{0.48\textwidth}{(f)}
          }
\caption{\label{fig:mass}}
\end{figure*}


\begin{figure*}[!htbp]
\gridline{\leftfig{Dust_snr=5_20201108.pdf}{0.48\textwidth}{(a)}
          \rightfig{Calibration_Dust_snr=5_20201108.pdf}{0.48\textwidth}{(b)}
          }
\gridline{\leftfig{SHAPz0_Dust_snr=5_20201108.pdf}{0.48\textwidth}{(c)}
          \rightfig{SHAPz2_Dust_snr=5_20201108.pdf}{0.48\textwidth}{(d)}
          }
\gridline{\leftfig{Epis_z0_Dust_snr=5_20201108.pdf}{0.48\textwidth}{(e)}
          \rightfig{Epis_z2_Dust_snr=5_20201108.pdf}{0.48\textwidth}{(f)}
          }
\caption{\label{fig:dustmass}}
\end{figure*}


\begin{figure*}[!htbp]
\gridline{\leftfig{Z_snr=5_20201108.pdf}{0.48\textwidth}{(a)}
          \rightfig{Calibration_Z_snr=5_20201108.pdf}{0.48\textwidth}{(b)}
          }
\gridline{\leftfig{SHAPz0_Z_snr=5_20201108.pdf}{0.48\textwidth}{(c)}
          \rightfig{SHAPz2_Z_snr=5_20201108.pdf}{0.48\textwidth}{(d)}
          }
\gridline{\leftfig{Epis_z0_Z_snr=5_20201108.pdf}{0.48\textwidth}{(e)}
          \rightfig{Epis_z2_Z_snr=5_20201108.pdf}{0.48\textwidth}{(f)}
          }
\caption{\label{fig:metallicity}}
\end{figure*}


\begin{figure*}[!htbp]
\gridline{\leftfig{SFR_snr=5_20201108.pdf}{0.48\textwidth}{(a)}
          \rightfig{Calibration_sfr_snr=5_20201108.pdf}{0.48\textwidth}{(b)}
          }
\gridline{\leftfig{SHAPz0_sfr_snr=5_20201108.pdf}{0.48\textwidth}{(c)}
          \rightfig{SHAPz2_sfr_snr=5_20201108.pdf}{0.48\textwidth}{(d)}
          }
\gridline{\leftfig{Epis_z0_sfr_snr=5_20201108.pdf}{0.48\textwidth}{(e)}
          \rightfig{Epis_z2_sfr_snr=5_20201108.pdf}{0.48\textwidth}{(f)}
          }
\caption{\label{fig:sfr}}
\end{figure*}


\iffalse
\begin{figure*}[!htb]
\gridline{\fig{Barplot_Mass_snr=5_20201101.pdf}{0.98\textwidth}{(a)}}
\gridline{\fig{Barplot_Mass_snr=5_20201101.pdf}{0.98\textwidth}{(b)}}
\gridline{\fig{Barplot_Mass_snr=5_20201101.pdf}{0.98\textwidth}{(c)}}
\gridline{\fig{Barplot_Mass_snr=5_20201101.pdf}{0.98\textwidth}{(d)}}
\caption{b}
\label{fig:stackedbarplots}
\end{figure*}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5555
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{figure*}[!htbp]
\gridline{\fig{Mass_snr=5_20201015.pdf}{0.48\textwidth}{(a)}
          \fig{Mass_snr=5_20201015.pdf}{0.48\textwidth}{(b)}
          }
\caption{\emph{Top panels:} Two dimensional kernel density estimate (KDE) plots of the means of galaxy properties. Blue and orange are the predicted means from \textrm{Prospector} using the non-parametric star formation history (SFH) model and \textrm{mirkwood}, v/s the true galaxy properties,respectively. %The dashed $y=x$ line indicates the ground truth values of the respective galaxy properties in both columns.
We also show three metrics to quantitatively compare results -- these are the normalized root mean squared error, the normalized mean absolute error, and the normalized bias error (Section ()). As  can be clearly seen, \textrm{mirkwood} significantly outperforms non-parametric fitting. \emph{Middle panels:} Bar plots comparing the quality of predicted error bars from non-parametric SED fits, \textrm{mirkwood}, and \textrm{mirkwood} post-processed using CRUDE calibration, in orange, green, and blue, respectively. For each of the three predictions, the top, lighter bars plot the interval sharpness, quantifying the `tightness' of predicted error bars. The lower, darker bars show the fraction of ground-truth galaxy values lying within $1 \sigma$ of their respective predicted error bars; see Section () for their precise definitions. A perfectly sharp set of predictions has IS and ECE of () and 0, respectively. Two things are immediately apparent: \textrm{mirkwood} significantly outperforms \textrm{Prospector}, and calibrating \textrm{mirkwood's} predictions is worth the extra compute time. \emph{Bottom panels:} Feature importance plots, comparing the relative importance of each of the 31 filters in predicting the two galaxy properties. SHAP values $>0$ indicate galaxy property values (mass for (a) and dust mass for (b)) greater than their means in their respective training sets, while red and blue respectively signify high and low flux values.}%We also highlight the importance of chaining models to account for dependenceFor each of the seven subplots, values predicted by mirkwood are plotted on the y-axis, while ground-truth values are on the x-axis. \textbf{(a):} Galaxy mass, in units of M$_{\odot}$. \textbf{(b):} From left to right: dust mass in units of M$_{\odot}$, gas phase metallicity in units of solar metallicity, and star formation rate in units of $\frac{M_{\odot}}{\textrm{year}}$. \textbf{(c):}}
\label{fig:mass,dustmass,snr5}
\end{figure*}

\begin{figure*}[!htb]
\gridline{\fig{Mass_snr=5_20201015.pdf}{0.48\textwidth}{(a)}
          \fig{Mass_snr=5_20201015.pdf}{0.48\textwidth}{(b)}
          }
\caption{b}%We also highlight the importance of chaining models to account for dependenceFor each of the seven subplots, values predicted by mirkwood are plotted on the y-axis, while ground-truth values are on the x-axis. \textbf{(a):} Galaxy mass, in units of M$_{\odot}$. \textbf{(b):} From left to right: dust mass in units of M$_{\odot}$, gas phase metallicity in units of solar metallicity, and star formation rate in units of $\frac{M_{\odot}}{\textrm{year}}$. \textbf{(c):}}
\label{fig:met,sfr,snr5}
\end{figure*}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\sc Prospector} and {\sc mirkwood} are given the same information in order to infer galaxy properties. This includes broadband photometry in $35$ bands with 5\%, 10\%, and 20\% Gaussian uncertainties (respectively SNRs = 20, 10, and 5). We present here the results from both methods for several galaxy properties including stellar mass, dust mass, star formation rate averaged over the last 100 Myr (SFR$_{100}$), and stellar metallicity.

In Figures \ref{fig:redshift} through \ref{fig:sfr}, we present {\sc mirkwood's} predictions when trained on the full dataset comprising of simulations from {\sc Simba}, {\sc Eagle}, and {\sc IllustrisTNG}, at both z=0 and z=2, for SNR=5\footnote{Corresponding plots for SNR=10 and SNR=20 are available online at \url{https://github.com/astrogilda/mirkwood}}. The training set contains 33,586 samples, and we use stratified 5-fold cross-validation (see Section \ref{sec:methods_proposed_method} for details on implementation) to split it into train and test sets. After making predictions on all test splits, we collate the results, thus successfully making predictions on all 33,586 samples. Each predicted output for a physical property contains three values -- the mean $\mu$, the aleatoric uncertainty $\sigma_{\rm a}$, and the epistemic uncertainty $\sigma_{\rm e}$. The first type of uncertainty quantifies the inherent noise in the data, while the second quantifies the confidence of the model in the training data (see Section \ref{sec:methods_uncertainty} for detailed description). The results from traditional SED fitting are a subset of the total training data -- for galaxies at z=2, we only fit samples from {\sc Simba} due to computational budget constraints. Thus this dataset consists of 14,258 samples -- 12,287 from all three simulations at z=0, and the rest from {\sc Simba} at z=2. We present a brief overview of the data sets in Table \ref{tab:datasetsummary}.

In subplots (a) of Figures \ref{fig:redshift} through \ref{fig:sfr}, we plot the recovered physical properties from {\sc mirkwood} and {\sc prospector} against the true values from the simulations for each of the five modeled properties: redshift, stellar mass, dust mass, metallicity, and star formation rate. In each case, the blue contours represent the physical properties derived from traditional SED fitting, while the orange points denote the results from {\sc mirkwood}. Without exception, {\sc mirkwood} provides superior predictions, as evidenced both by a visual inspection, and via a more quantitative approach by using three different metrics (detailed in Section \ref{sec:methods_metrics}). 

%\red{I know you're trying to be concise here, but you probably need to explain this to a dolt astronomer who knows very little about ML [like me...] and walk the reader through carefully.  There's no point in plotting it if an astronomer can't understand it (and, I don't think from this explanation they will be able to).  Remember the audience is not ML: it's an OIR observer who may switch from SED fitting to this model.}
In subplots(b), we plot `calibration diagrams' \citep{crude_probability_calibration}. %\red{Desika leaving off here please leave this note so i know where to re-join}
On the y-axis are the inverse-CDFs (cumulative distribution functions) for predictions from both {\sc mirkwood} and {\sc Prospector}. These are commonly used in ML literature -- the plotting function takes as input a vector consisting of the ground truth value, predicted mean, and predicted standard deviation, and outputs a value between 0 and 1 (see \cite{probability_calibration1} for detailed instructions on constructing these diagrams). We repeat this for all samples in the test set $\mathcal{D_{TEST}}$, sort the resulting vector in ascending order, and plot the curve on the y-axis. For {\sc mirkwood}, the uncertainty used is $\sigma_{\rm a}$, while {\sc Prospector} does not differentiate between the two types of uncertainties and outputs only a single value per galaxy sample. A 1:1 line on this curve indicates a perfectly calibrated set of predictions, with deviations farther from it indicative of poorer calibration. Both visually and quantitatively by using the two probabilistic metric (Section \ref{sec:methods_metrics}) average coverage error and interval sharpness, we ascertain that {\sc mirkwood} outperforms traditional SED fitting.

In subplots (c) and (d), we plot the SHAP summary plots for samples in $\mathcal{D_{TEST}}$, for redshifts 0 and 2 respectively. We explain in detail how SHAP values are calculated in Section \ref{sec:shapley_values}. In brief, for a given filter (dotted vertical lines in subplots (c) and (d)), an absolute value farther from 0 denotes a larger impact of that feature in affecting the model outcome. SHAP value can thus be thought of as a type of sensitivity -- it controls how reactive the output is to changes in the input (here flux in the filter). Red and blue indicate high and low ends of values per feature/filter. Thus for a given feature, SHAP values $> 0$ with a red hue indicate that the galaxy property increases as that feature increases. Similarly, SHAP values $> 0$ with a blue hue indicate that the galaxy property decreases as the feature value decreases. As an example, in panel (c) of Figure~\ref{fig:mass}, the largest correlations with the $M^{\star}$ of a galaxy are, quite naturally, the $\sim 1-2 \mu$m range.% \red{desika leaving off here}

In subplots (e) and (f), we plot epistemic errors from {\sc mirkwood} against the most informative feature derived from their respective subplots (c) and (d). Over-plotted on these are the scaled histograms for the same feature, from the training and test sets, at these two redshifts\footnote{To be able to plot values differing by orders of magnitude on the same plot, we convert both the $x$ and $y$ axis to log-scale; the addition of the unit vector ensures that small values remain close to 0 after conversion and do not turn negative.}. $\sigma_{\rm e}$ informs us of the degree of confidence the model has in its predictions in a given part of the parameter space; by plotting it against the most informative filter derived from the SHAP plot, we can get a first order visual insight into the model's decision making process. In all Figures from \ref{fig:redshift} through \ref{fig:sfr}, we see a general trend that epistemic uncertainties increase when when the informative features become sparse, just as we would intuitively expect.

In Table \ref{tab:stackedbartable}, we delineate all five metrics from Section \ref{sec:methods_metrics} to quantitatively compare {\sc mirkwood}'s performance with that of traditional SED fitting, across different levels of noise. As we would expect, the results from both models improve with increasing SNR. Across every metric and galaxy property, {\sc mirkwood} emerges as the clear winner. We also note that the difference in their relative performances increases with increasing noise level. Below a certain SNR, traditional SED fitting stops producing meaningful results (as can also be seen clearly from subplots (a) in Figures \ref{fig:redshift} through \ref{fig:sfr}
), whereas our ML-based approach is still able to extract signal from the noisy data.

\iffalse
\subsection{Redshift}\label{sec:results_redshift}
We see in Figure \ref{fig:redshift}(a) that even with low quality SNR=5 photometric data, {\sc mirkwood} is able to recover redshifts almost perfectly. Figure \ref{fig:redshift}(b), however, paints a slightly different picture. Instead of getting an ideal 1:1 plot, we get a horizontal curve -- this is because for all samples used in this paper, the probability density function (PDF) for each of the galaxy of the fact that for each of the xxx samples in $\mathcal{D_{TEST}}$, the ground truth redshift effectively lies smack-dab at the median of the Gaussian distribution constructed using predicted $\mu$ and $\sigma_{\rm a}$. In other words, our predicted uncertainties are too small. We suspect this is because for this binary sample, our assumption of Gaussianity is broken, and perhaps a more suitable distribution is the Bernoulli. We leave this to future work.

In Figures \ref{fig:redshift}(c) and (d) we see that the most predictive bands are in the UV and NIR to MIR. Since we have broken up $\mathcal{D_{TEST}}$ into two subsets based on the redshift $z$, each of the two plots (c) and (d) contain only 1 $z$ value, and hence the SHAP values are biased in the way they are.
%\green{(Desika: can we explain why the given bands are important for redshift?)}

\subsection{Stellar Mass}\label{sec:results_stellarmass}
We see in Figure \ref{fig:mass}(a) that {\sc mirkwood} is able to almost perfectly recreate the true stellar mass, whereas traditional SED fitting performs very poorly. We emphasize that the values plotted on the $y$-axis are the predicted means from both the models -- this means that even without accounting for uncertainties, the predicted means from {\sc Prospector} are untrustworthy on account of their large spread. In Figure \ref{fig:mass}(b) we see that our proposed model is almost perfectly calibrated, whereas {\sc Prospector} using the non-parametric SFH formulation of \cite{leja2017deriving} is under-confident with its predictions at levels below $\sim 0.3$, and extremely over-confident immediately after. 

Figures \ref{fig:mass}(b) and (c) provide us several pieces of information. We immediately see that the most information bands are $J$, $H$, and $K$, as expected. Note the disparity between the ranges of SHAP values. At z=0, fluxes have a biased effect on prediction of stellar mass -- a lack of flux (blue color) decreases predicted mass slightly, whereas an excess of flux increases mass much more rapidly. On the other hand, at z=2, the impact of the most informative bands is even with respect to direction of prediction. We also note that at z=2 NIR features are considerably more relevant, which is also something we would expect.

\subsection{Impact of SNR}\label{sec:results_SNR}
In Table \ref{tab:stackedbartable} we compare {\sc mirkwood}'s predictions with {\sc Prospector}'s, as a function of noise in the input data. We can clearly see that our proposed model retains its edge even at extremely high levels of noise.
\fi

\iffalse
In Figure (), we compare \textrm{mirkwood}'s performance on retrieving $\log (M^{\star}/M_{\odot})$ values (median in the top panel, and $16^{\rm th}$ and $84^{\rm th}$ percentiles in the middle panel) with that of traditional SED fitting using the non-parametric SFH of \cite{lower_stellar_mass}. The input SEDs have been artificially introduced with Gaussian noise such that their signal-to-noise ratio is 5. As can be seen both visually and quantitatively via the various deterministic and probabilistic metrics, our performance is almost an order of magnitude better. In the bottom panel, we see that \textrm{mirkwood}

In the absence of noise, our performance on log10 Mstar
is reasonable for individual galaxies, with overall biases
a few percent or less and uncertainty of the order of 10
per cent, as shown in Table 1. The overall distribution
is well reproduced by eye, and likely well reproduced
enough for scientific applications, although distribution
similarity tests such as the K-S test indicate that the
distributions are statistically different. The error as a
function of galaxy parameter in Fig. 4 demonstrates that
we can train the networks well where there is a high
density of points, but we have increased errors towards
the tails of the distribution.

We now compare our results to stellar mass measurements of mock catalogs. Mobasher et al. (2015) performed a comprehensive study to estimate uncertainties
and sources of bias in measuring physical parameters in
galaxies. A number of different tests were performed,
based on different initial parameters and codes. Here
we adopt TEST-2A as our benchmark, as it is closest to
our sample. TEST-2A used semianalytic models with
a diversity of star formation histories and other parameters, and as with our semianalytic models, used measurements in CANDELS filter bands as their data set.
We note that TEST-2A used more CANDELS bands
than our measurement here: 13 instead of 8, including U-band, K-band, and Spitzer infrared data in addition to the Hubble optical and near-infrared bands we
use, and excluding the F184W (ACS) filter that we use.
Comparing to the distribution of biases and uncertainties returned by the individual methods in Mobasher
et al. 2015, we find that we easily improve on the bias
and have competitive uncertainty in our measurements.
However, we expect to have lower bias: different assumptions of initial mass functions, star formation rates,
etc were found by Mobasher et al. 2015 to be a source
of systematic offsets between different codes, adding a
constant bias to every galaxy, whereas we are implicitly
assuming the same initial mass function and star formation rate since our samples are drawn from the same
mock catalog. Our templates also have varying amounts
of dust and varying metallicities, the lack of which has
also been found to bias stellar mass estimates (Mitchell
et al. 2013).
We repeat the analysis with pseudo observational error, either matched to the full uncertainty distribution
or matched to the uncertainty distribution of galaxies
which have at least a 5σ-detected flux measurement in
each band. We show only the best-performing input column set from the noise-free case, after checking that this
column choice still performs best when error is added.
This additional simulated observational noise causes an
increase in bias and a large increase in uncertainty, visible in the right-hand plots of Fig. 4. However, the average bias of −0.019 dex is still smaller by an order of
magnitude than any of the biases from Mobasher et al.
(2015) (with the same caveat about correct implicit assumptions), and the uncertainty only a little worse than
the maximum uncertainty from that comparison, 0.203
dex instead of 0.183 dex.

\subsection{Dust Mass}\label{sec:results_dustmass}

\subsection{Stellar Metallicity}\label{sec:results_stellarmet}
As with stellar mass, we find good performance from
our metallicity-predicting neural networks, with small
biases and order 10 per cent uncertainty, as shown in
Table 2 and Fig. 5. The overall predicted distribution
is somewhat more skewed from the original distribution
than in the stellar mass case, though again we perform
well where the density of training points is high. As with
stellar mass, we perform worse when noise is included,
but not by a significant amount: an increase of bias by a
factor of 2 and uncertainty by a factor of 3. This uncertainty, of 0.2 dex in the full-noise case, is larger than the
convolutional neural network machinery of Wu & Boada
(2018), who obtained 0.08 dex uncertainty, albeit using
substantially more data (3-color 128x128 pixel cutouts,
not eight measured magnitudes) and brighter and lowerredshift galaxies (brighter than 25th magnitude). We
obtain a similar result to theirs in that low-metallicity
galaxies have systematically high metallicity predictions
in the presence of noise.
This good performance on metallicity requires some
discussion. Metallicity is typically the hardest of these
properties to measure by traditional methods so it is
surprising that we are able to do well. The dominant
component of our performance is driven by the relationship between metallicity and stellar mass. There is a
strong relationship between these quantities in data and
in simulation (Lu et al. 2014, and references therein),
and in practice the fact that we can fit stellar mass well
means that most of our prediction of metallicity comes
from the ability of the network to learn the Mstar −Zstar
connection and to predict Mstar from the photometry, as
can be seen by the similar shape of the bias-parameter
curves in the noisy right-hand columns of in Fig. 4 and
Fig. 5. That cannot be the full picture–metallicity performs best when we use colors alone, while stellar mass
performs best when we use both magnitudes and colors–
but it is a significant contributor to our good results.

To illustrate this, we fit a simple quadratic equation to
the log10 Mstar − log10 Zstar relationship in the simulations to predict a metallicity for each galaxy assuming
no noise, and then we check how much improvement we
get from the noise-free neural network when compared
to this simple Mstar-based prediction. Fig. 6 shows a
2-D histogram of this improvement, with points above 0
being an improvement on the polynomial fit, and points
below 0 having an increased bias. The bulk of our neural
network predictions do improve on the simple model, by
1-2σ, but given that our data spans more than 2 orders
of magnitude, an improvement of 0.1-0.2 dex indicates
that the simple stellar mass-metallicity relationship can
explain a good fraction of our predicted metallicities.
The additional improvement is also suggested by the
fact that the metallicity network performs better without magnitudes, while the stellar mass network performs
better with them, meaning that the metallicity network
must be learning different information than stellar mass
alone. Still, this effect suggests that, for any method,
if metallicity is not well-constrained by the data, using
a stellar mass-based prior with appropriate uncertainty
may produce adequate results.



\subsection{Instantaneous Star Formation Rate}\label{sec:results_sfr}
For the star formation rate, we have slightly higher
bias and uncertainty. The bias of −0.053 dex corresponds to a 12 percent error in linear space, visible in
the histogram of Fig. 7 as the blue prediction histogram
peaking slightly higher than the true distribution in red.
Much of the uncertainty is contributed by points with
very low star formation rates. Fig. 7 shows the performance as a function of predicted star formation rate as
well as a histogram of true and predicted values.

\subsection{Instantaneous Star Formation Rate}\label{sec:results_redshift}
None of these networks used redshift as an input, but
template-fitting methods generally require it (Mobasher
et al. 2015). Do our results improve if we add redshift
as an input to the networks trained on the other galaxy
properties? We take the best-performing input column
set for stellar mass, metallicity, and star formation rate,
and add redshift as an input. The results are summarized in Table 4. For stellar mass and star formation
rate, the mean bias and the uncertainty both improve.
However, the improvement in the uncertainty is generally small, and the change in bias is less than the uncertainty for all three galaxy properties. This is an encouraging result, as it means we can achieve good accuracy
without needing to supplement our data with spectroscopic redshifts.
\fi


\begin{table*}
    \caption{Comparative performance of {\sc mirkwood} v/s {\sc Prospector} across different noise regimes. The five metrics are the normalized root mean squared error (NRMSE), normalized mean absolute error (NMAE), normalized bias error (NBE), average coverage error (ACE), and interval sharpness (IS). In any given cell, the tuple of values consists of the metric of interest from {\sc mirkwood} and {\sc Prospector}, respectively. A value of `nan' represents lack of predictions from {\sc Prospector}. Since traditional SED fitting hasn't been used to derive the redshift, the second values in all tuples in the `Redshift' field are `nan's. Similarly, we do not have predicted error bars from {\sc Prospector}for dust mass, hence ACE and IS values corresponding to this property are `nan's.}
    \label{tab:stackedbartable}
    \centering
    \begin{tabular}{ccccccc}
    \toprule
    & SNR &  NRMSE &  NMAE & NBE & ACE & IS \\ \tableline
    & 5  &  (0.0, nan) &  (0.0, nan) &  (-0.0, nan) &  (0.317, nan) &  (0.0, nan) \\
    Redshift & 10 &  (0.0, nan) &  (0.0, nan) &  (-0.0, nan) &  (0.317, nan) &  (0.0, nan) \\
    & 20 &  (0.0, nan) &  (0.0, nan) &   (0.0, nan) &  (0.317, nan) &  (0.0, nan) \\ \tableline
    & 5  &  (\textbf{0.198}, 1.003) &  (\textbf{0.123}, 1.091) &  (\textbf{-0.042}, -0.528) &  \textbf{(-0.002}, -0.497) &  (\textbf{0.001}, 0.005) \\
    Mass & 10 &    (\textbf{0.165}, 1.0) &  (\textbf{0.118}, 1.088) &  (\textbf{-0.035}, -0.518) &  (\textbf{-0.021}, -0.502) &  (\textbf{0.001}, 0.004) \\
    & 20 &  (\textbf{0.155}, 1.002) &  (\textbf{0.115}, 1.117) &  (\textbf{-0.041}, -0.479) &  (\textbf{-0.066}, -0.482) &  (\textbf{0.001}, 0.033) \\ \tableline
    & 5  &   (\textbf{0.48}, 0.996) &  (\textbf{0.339}, 0.998) &  (\textbf{-0.219}, -0.905) &   (\textbf{0.003}, nan) &  (\textbf{0.001}, nan) \\
    Dust Mass & 10 &  (\textbf{0.456}, 0.996) &  (\textbf{0.332}, 0.998) &  (\textbf{-0.209}, -0.905) &  (\textbf{-0.033}, nan) &  (\textbf{0.001}, nan) \\
    & 20 &  (\textbf{0.475}, 1.263) &  (\textbf{0.336}, 1.212) &  (\textbf{-0.215}, -0.679) &  (-0.076, nan) &  (0.001, nan) \\ \tableline
    & 5  &  (\textbf{0.062}, 0.544) &   (\textbf{0.06}, 0.478) &  (\textbf{-0.011}, -0.297) &  (\textbf{-0.024}, 0.046) &  (\textbf{0.041}, 0.301) \\
    Metallicity & 10 &  (\textbf{0.058}, 0.534) &  (\textbf{0.055}, 0.464) &   (\textbf{-0.01}, -0.275) &  (\textbf{-0.032}, 0.041) &  (\textbf{0.036}, 0.295) \\
    & 20 &  (\textbf{0.056}, 0.547) &  (\textbf{0.052}, 0.487) &   (\textbf{-0.01}, -0.229) &  (\textbf{-0.063}, 0.036) &  (\textbf{0.032}, 0.302) \\ \tableline
    & 5  &  (\textbf{0.241}, 0.907) &   (\textbf{0.205}, 0.99) &  (\textbf{-0.069}, -0.687) &  (\textbf{0.074}, -0.557) &  (7.314,\textbf{ 0.001}) \\
    SFR & 10 &   (\textbf{0.329}, 0.91) &  (\textbf{0.226}, 0.992) &   (\textbf{-0.09}, -0.686) &  (\textbf{0.048}, -0.564) &  (\textbf{1.937}, 0.001) \\
    & 20 &  (\textbf{0.277}, 1.988) &  (\textbf{0.215}, 2.911) &   (\textbf{-0.078}, 1.437) &  (\textbf{0.035}, -0.547) &    (\textbf{0.006}, 0.2) \\ \tableline
    \end{tabular}
\end{table*}


==> calibration.tex <==
\subsection{Calibration of Probabilities}\label{sec:calibration}

Above, we have described the procedure for obtaining both aleatoric and epistemic errors. However, not all errors are created equal -- in practice, most uncertainty estimates often fail to capture the underlying data distribution \citep{lakshminarayanan_probability_calibration0, probability_calibration1, crude_probability_calibration}. For example, a 95 \% confidence interval generally does not contain the true outcome 95\% of the time (see Figure ()). When this happens, the model is said to be \emph{miscalibrated}. This is typically caused by model overconfidence, if the model is not powerful enough to map the right probability to its confidence interval. Calibration, or lack thereof, is also a function of the loss function the model is trained to minimize. Negative log-likelihood, the loss function we train \textsc{mirkwood} to minimize in this paper (see Section()), is known to result in over-confident predictions \citep{measuring_calibration_in_deep_learning}. Thus, we need to \emph{post hoc} correct the uncalibrated probabilities our model outputs.

Here, we use the CRUDE method of \cite{crude_probability_calibration} to re-calibrate our model's predictions \emph{post-hoc}. CRUDE ensures that not only are the post-processed predictions calibrated, but that they are also \emph{sharp} \citep{measuring_calibration_in_deep_learning}. Sharpness refers to the concentration of the predictions.  The more peaked (the sharper) the predictions are, the better (provided it is not at the expense of calibration).

%Noting that, in practice, most uncertainty estimates are over-confident when estimating the prediction uncertainty \citep{lakshminarayanan_probability_calibration0, probability_calibration1, crude_probability_calibration},  we use the CRUDE method \cite{crude_probability_calibration} to re-calibrate our model's predictions \emph{post-hoc}. CRUDE ensures that not only are the post-processed predictions calibrated, but that they are also \emph{sharp} \citep{measuring_calibration_in_deep_learning}. Sharpness refers to the concentration of the predictions.  The more peaked (the sharper) the predictions are, the better (provided it is not at the expense of calibration).

%Here, we use the CRUDE method of \cite{crude_probability_calibration} to \emph{post-hoc} re-calibrate our model's predictions. This method ensures that not only are the post-processed predictions \emph{calibrated}, but that they are also \emph{sharp}. While calibration ensures that each percentile matches the fraction of values observed below the predictions of that percentile \citep{measuring_calibration_in_deep_learning}, sharpness refers to the concentration of the predictions--the more concentrated the predictive distributions are, the sharper the forecasts, and the sharper the better (provided it is not at the expense of calibration). \cite{crude_probability_calibration} show that CRUDE not only results in better calibrated predictions compared to previously proposed methods \textbf{get citations from the crude paper}, but also sharper predictions.



==> filters_table.tex <==
\begin{table*}
\begin{tabular}{llc|llc}
\tableline
Instrument    & Filter & Effective Wavelength (AA) & Instrument     & Filter & Effective Wavelength (AA) \\ \tableline
GALEX         & FUV    & 1549                      &                & F070W  & 7007                                          \\
              & NUV    & 2304                      &                & F090W  & 8980                                          \\ \cline{1-3}
              & F275W  & 2720                      & JWST/NIRCam    & F115W  & 11487                                         \\
              & F336W  & 3359                      &                & F150W  & 14942                                         \\
              & F475W  & 4732                      &                & F200W  & 19791                                         \\
              & F555W  & 5234                      &                & F277W  & 27466                                         \\ \cline{4-6} 
              & F606W  & 5780                      &                & F560W  & 56151                                         \\
HST/WFC3      & F814W  & 7977                      &                & F770W  & 75911                                         \\
              & F105W  & 10431                     &                & F1000W & 99230                                         \\
              & F110W  & 11203                     & JWST/MIRI      & F1130W & 127677                                        \\
              & F125W  & 12364                     &                & F1280W & 113035                                        \\
              & F140W  & 13735                     &                & F1500W & 150078                                        \\
              & F160W  & 15279                     &                & F1800W & 179390                                        \\ \tableline
Spitzer/IRAC  & Ch1    & 35075                     & Spitzer/MIPS   & 24 um  & 232096                                        \\ \tableline
              & Blue   & 689247                    &                & PSW    & 2428393                                       \\
Herschel/PACS & Green  & 979036                    & Herschel/SPIRE & PMW    & 3408992                                       \\
              & Red    & 1539451                   &                & PLW    & 4822635                                       \\ \tableline
\end{tabular}


\caption{Table of the 33 filters used to extract photometry from the synthetic {\sc powderday} spectra.}
\end{table*}\label{table:filters}






==> interaction_effects.tex <==
\subsection{SHAP Interaction Effects}\label{sec:shap_interaction}
See the Tree SHAP paper for more details, but briefly, SHAP interaction values are a generalization of SHAP values to higher order interactions.

The interaction effect is the additional combined feature effect after accounting for the individual feature effects.

This formula subtracts the main effect of the features so that we get the pure interaction effect after accounting for the individual effects. We average the values over all possible feature coalitions S, as in the Shapley value computation. When we compute SHAP interaction values for all features, we get one matrix per instance with dimensions M x M, where M is the number of features.

How can we use the interaction index? For example, to automatically color the SHAP feature dependence plot with the strongest interaction:



==> intro_to_ml.tex <==
\subsection{What is Machine Learning?}\label{sec:methods_intro_to_ml}
\red{NO TEXT HERE?}

==> metrics_for_prob_preds.tex <==
\subsection{Metrics for Probabilistic Predictions}
Probabilistic predictions are assessed by constructing Prediction Intervals (PI) and using corresponding PI evaluation criteria. In this work, we adopt the following four PI criteria:
\begin{itemize}
    \item Average Coverage Area. ACE is an indicator to appraise the reliability of prediction interval, which has the following equation:
    \begin{align}
        \mathrm{ACE}_{\alpha}=\frac{1}{n} \sum_{i=1}^{n} c_{i} \times 100 \%-100 \cdot(1-\alpha) \%,
    \end{align}
    where $c_i$ is the indicative function of coverage and its calculation equation is as:
    \begin{align}
        c_{i}=\left\{\begin{array}{l}
1, y(i) \in\left[l_{\alpha}(i), u_{\alpha}(i)\right] \\
0, y(i) \notin\left[l_{\alpha}(i), u_{\alpha}(i)\right]
\end{array}\right.
    \end{align}
    \item Prediction Interval Normalized Average Width (PINAW):
    \begin{align}
        \mathrm{PINAW} = \frac{\sum_{i=1}^n U_i - L_i}{nr},
    \end{align}
    where $r = y_{max} - y_{min}$. PINAW is the mean of PI widths normalized by the range of testing targets.
    \item Interval Sharpness (IS):
    \begin{align}
        \mathrm{IS}_{\alpha}=\frac{1}{n} \sum_{t=1}^{n}\left\{\begin{array}{ll}
-2 \alpha\Delta_{\alpha}(i)-4\left[l_{\alpha}(t)-y(t)\right], & y(t)<l_{\alpha}(t) \\
-2 \alpha\Delta_{\alpha}(i)-4\left[y(t)-u_{\alpha}(t)\right], & y(t)>u_{\alpha}(t) \\
-2 \alpha\Delta_{\alpha}(i), & \mathrm{otherwise}\end{array}\right.
    \end{align}
    where $\Delta_{\alpha}(i) = u_{\alpha}(i)-l_{\alpha}(i)$.
    \item Continuous Ranked Probability Score (CRPS):
    \begin{align}
        \mathrm{CRPS}=\int_{-\infty}^{\infty}(F(y)-\mathbb{1}(y-x))^{2} d y,
    \end{align}
    where $F$ is the cumulative distribution function (CDF) associated with the probabilistic forecast, and $\mathbb{1}$ is the Heaviside step function.
\end{itemize}
From the equation of ACE, a value close to zero denotes the high reliability of prediction interval. As an infinitely wide prediction interval is meaningless, IS is another indicator contrary to the coverage rate of interval, which measures the accuracy of probabilistic forecasting. $\mathrm{IS}_{\alpha}$ is always $<0$; a great prediction interval obtains high reliability with a narrow width, which has a small absolute value of IS. PINAW is the mean of PI widths normalized by the range of testing targets. Our goal is to ensure that PI is not too wide, since that would make it useless as a metric. The CRPS is a measure of the integrated squared difference between the cumulative distribution function of the forecasts and the corresponding cumulative distribution function of the
observations. It CRPS generalizes the mean absolute error (MAE), and reduces to it if the forecast is deterministic. It simultaneously considers the reliability and sharpness, and is a commonly used metric to evaluated the performance of the predicted conditional PDF. Note that CRPS is the only metric that uses the raw predicted PDF, and not the predicted intervals obtained by using Equation ().



==> observational_pred.tex <==
\section{Observational Predictions}

-apply mirkwood and prospector to a sample of observations?


==> outline.tex <==
\section{Outline}

\begin{itemize}
    \item Intro
    \begin{itemize}
        \item Introduce SED fitting
        \item highlight that this is a publicly available package that will be continuously updated
        \item other stuff (?)
    \item flow into galaxy properties inferred using ML + crash course in ML
    \end{itemize}
    \item Related Work/State-of-the-art
    \begin{itemize}
        \item Bayesian fitting codes--Prospector
        \item emphasize cpu hrs per fit
        \item \textbf{plots}
    \item prospector for traditional SED fit comparison
    \end{itemize}
    \item Data
    \begin{itemize}
        \item brief introduction to SIMBA, EAGLE, TNG.
        \item differences between them.
        \item process of generating galaxies from sims
        \item process of generating SEDs from galaxies.
        \item galaxy properties we are using
        \item emphasize we are only using z=0 to show proof-of-concept.
    \end{itemize}
    \item Methods
    \begin{itemize}
        \item very brief introduction to popular tree based models, including ngboost
        \item introduce ensembling
        \item introduce automl
        \item errors--epistemic vs aleatoric
        \item metrics--deterministic and probabilistic
        \item shapley values, and SHAP.
        \item \textbf{plot}: schematic overview of process
    \end{itemize}
    \item Results
    \begin{itemize}
        \item galaxy physical properties (mass, SFR, dustmass, Z): mirkwood vs. trad. SED
        \item \textbf{3 plots x 4} train on sim1, predict on other 2, for each property
        \item \textbf{plot x 4}: train on all 3. predict on all 3, for each property
        \item \textbf{plot x 4}: summary plot using mu, for each property
        \item \textbf{plot x 4}: summary plot using aleatoric sigma, for each property
        \item \textbf{plot x 4}: feature interaction plot using mu, for each property
        \item \textbf{plot x 4}: feature interaction plot using aleatoric sigma, for each property
        \item \textbf{plot}: for outliers
    \end{itemize}
    \item Discussion
    \begin{itemize}
        \item discussion on assumptions in mirkwood vs. assumptions in SED fitting
        \item other stuff
    \end{itemize}
    \item Differentiate super-learner from stacking (stacked-generalization)/blending, and cite papers for both
    \item Potential figure explaining stacking--https://machinelearningmastery.com/super-learner-ensemble-in-python/
    \item include that paper in bib that proves the importance of using 'max_samples' as a hyper-parameter
    \item \url{https://arxiv.org/pdf/2002.03578.pdf}
    \item \url{https://arxiv.org/pdf/1905.08996.pdf}
    \item \url{https://arxiv.org/pdf/1903.10457.pdf}
    \item \url{https://www.aanda.org/articles/aa/pdf/2019/02/aa33972-18.pdf}
    \item \url{https://ui.adsabs.harvard.edu/abs/2020IAUS..341...88A/abstract}
    \item \url{https://ui.adsabs.harvard.edu/abs/2005MNRAS.362...41G/abstract}
    
    %\item By training a meta-model on out-of-sample predictions of other models, the meta-model learns how to both correct the out-of-sample predictions for each model and to best combine the out-of-sample predictions from multiple models; actually, it does both tasks at the same time.
    %\item Each out-of-fold prediction will be a column for the meta-model input. We will collect columns from each algorithm for one fold of the data, horizontally stacking the rows. Then for all groups of columns we collect, we will vertically stack these rows into one long dataset with 500 rows and nine columns.
    %https://www.kaggle.com/flennerhag/ml-ensemble-scikit-learn-style-ensemble-learning
    %http://ml-ensemble.com/info/tutorials/advanced.html#model-selection-tutorial
    %
\end{itemize}


==> performance_metrics.tex <==
\subsection{Performance Metrics}\label{sec:methods_metrics}
As we have discussed, for each input sample {\sc mirkwood} outputs three values: $\mu$, $\sigma_{a}$, and $\sigma_{e}$. As the same time, for each input, {\sc Prospector} outputs two values: $\mu$, and $\sigma$. We quantify the performance of each model by comparing the predicted galaxy properties against the true ones known from simulations. We divide this task into two parts -- comparing just the predicted mean \emph{deterministic predictions} of each galaxy property with its ground truth value, and judging the quality of the entire predicted PDF  (probability distribution function; \emph{probabilistic predictions}) by comparing it against the ground truth value.

\subsubsection{Metrics for Deterministic Predictions}\label{sec:metrics_det}
For determining the `goodness' of the predicted means for the galaxy properties, we adopt the following three performance criteria:
\begin{itemize}
    \item Normalized root-mean-square error (RMSE):
    \begin{align*}
        \mathrm{NRMSE}=\sqrt{\frac{1}{n} \sum_{i=1}^{n}\left(\hat{\mu}(i)-Y(i)\right)^{2}}
    \end{align*}
    \item Normalized mean absolute error (NMAE):
    \begin{align*}
        \mathrm{NMAE}=\frac{1}{n} \sum_{i=1}^{n}\left|\hat{\mu}(i)-Y(i)\right|
    \end{align*}
    %\item Normalized mean absolute percentage error (NMAPE):
    %\begin{align}
    %    \mathrm{NMAPE}=\frac{1}{n} \sum_{i=1}^{n} \frac{\left|\tilde{y}(i)-y(i)\right|}{\max _{i \in 1, \mathrm{n}]} y(i)} \times 100 \%,
    %\end{align}
    \item Normalized bias error:
    \begin{align*}
        \mathrm{NBE} = \frac{1}{n} \sum_{i=1}^{n} \hat{\mu}(i)-Y(i)
    \end{align*}
\end{itemize}
where $Y(i)$ and $\hat{\mu}(i)$ are the true and predicted values of any of the five galaxy properties for the $i^{th}$ sample, while $n$ is the total number of samples. A perfect prediction would result in NRMSE, NMAE, and NBE of 0. These values can be seen in the top-left plots in Figures \ref{fig:mass} through \ref{fig:sfr}.

\subsubsection{Metrics for Probabilistic Predictions}\label{sec:metrics_prob}
Probabilistic predictions are assessed by constructing Confidence Intervals (CI) and using them in evaluation criteria. In this work, we adopt average coverage area (ACE) and interval sharpness (IS) as our metrics. $\alpha$ is the significance level -- the probability that one will mistakenly reject the null hypothesis when in fact it is true. Specifically, since in this paper we are interested in $+/- 1\sigma$ predictions (CI=68.2\%), we choose $\alpha = 1-\rm{CI} = 0.318$. For {\sc mirkwood} results, $\sigma = \sqrt{\sigma_{a}^2 + \sigma_{e}^2}$, while for {\sc Prospector} results, there is only one $\sigma$ per prediction. For a given sample $i$, if the prediction of any galaxy property, from either {\sc mirkwood} or {\sc Prospector}, is \{$\mu(i)$; $\sigma(i)$\}, then the lower and upper confidence intervals  $L_\alpha(i)$ and $U_\alpha(i)$ are given by $\mu(i) - \sigma(i)$ and $\mu(i) + \sigma(i)$, respectively. $l_\alpha(i)$ and $u_\alpha(i)$ correspond to the $u-$values for these: $l_\alpha(i) = 0.5 - \rm{CI}/2 = 0.159$, $u_\alpha(i) = 0.5 + \rm{CI}/2 = 0.841$. $y(i)$ corresponds to the $u-$value of the ground truth value $Y(i)$. If the predicted mean $\hat{\mu}(i)$ for a galaxy property exactly matches $Y(i)$, then $y_\alpha(i)=0.5$; if the predicted mean overshoots or undershoots the ground truth value, then $y_\alpha(i) > 0.5$ or $y_\alpha(i) < 0.5$, respectively.

\begin{itemize}
    \item Average Coverage Error (ACE): %ACE is an indicator to appraise the reliability of prediction interval, which has the following equation:
    \begin{align*}
        \mathrm{ACE}_{\alpha}=\frac{1}{n} \sum_{i=1}^{n} c_{\alpha}(i) \times 100 \%-100 \times(1-\alpha) \%,
    \end{align*}
    where $c_i$ is the indicative function of coverage:
    \begin{align*}
        c_{\alpha}(i)=\left\{\begin{array}{l}
1, Y(i) \in\left[L_{\alpha}(i), U_{\alpha}(i)\right] \\
0, Y(i) \notin\left[L_{\alpha}(i), U_{\alpha}(i)\right]
\end{array}\right.
    \end{align*}
    ACE is effectively the ratio of target values falling within the confidence interval to the total number of predicted samples.
    \item Interval Sharpness (IS):
    \begin{align*}
        \mathrm{IS}_{\alpha}=\frac{1}{n} \sum_{t=1}^{n}\left\{\begin{array}{ll}
-2 \alpha\Delta_{\alpha}(i)\\-4\left[l_{\alpha}(i)-y(i)\right], & y(i)<l_{\alpha}(t) \\
-2 \alpha\Delta_{\alpha}(i)\\-4\left[y(i)-u_{\alpha}(i)\right], & y(i)>u_{\alpha}(t) \\
-2 \alpha\Delta_{\alpha}(i), & \mathrm{otherwise}\end{array}\right.
    \end{align*}
    where $\Delta_{\alpha}(i) = u_{\alpha}(i)-l_{\alpha}(i) = 0.682$. As a reminder, corresponding to $+/- 1\sigma$ intervals, $\alpha=0.318$, $l_{\alpha}(i)=0.159$, and $u_{\alpha}(i)=0.841$.
\end{itemize}

From the equation of ACE, a value close to zero denotes the high reliability of prediction interval. As an infinitely wide prediction interval is meaningless, IS is another indicator contrary to the coverage rate of interval, which measures the accuracy of probabilistic forecasting. $\mathrm{IS}_{\alpha}$ is always $<0$; a great prediction interval obtains high reliability with a narrow width, which has a small absolute value of IS. 
%\textbf{MAKE SURE THIS ABOVE PARA ISN'T PLAGIARIZED; I HAVE A VAGUE RECOLLECTION OF COPYING SOME BITS FROM SOMEWHERE WITH THE INTENTION OF LATER MODIFYING THEM.}


\begin{figure*}
    \centering
    \includegraphics[width=0.98\textwidth]{chaining.pdf}
    \caption{Chained multi-output regression. From left to right, we train models to sequentially predict galaxy redshift, stellar mass, dust mass, stellar metallicity, and SFR$_{100}$. At the first step, we train {\sc mirkwood} on fluxes (as input) and redshift (as output) in the training set $\mathcal{D_{TRAIN}}$, and use it to predict redshifts for samples in the test set ($\mathcal{D_{TEST}}$) using their respective flux values as inputs. In the second step, we append the true true redshifts of samples in $\mathcal{D_{TRAIN}}$ to with their fluxes, and append the predicted redshifts of the samples in $\mathcal{D_{TEST}}$ to their fluxes. A new model is then trained on the extended training set, and used to predict stellar mass for samples in the test set. We continue thus until all five properties have been successfully predicted for all samples in the original $\mathcal{D_{TEST}}$.}
    \label{fig:chaining}
\end{figure*}



==> proposed_method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.80\textwidth]{mirkwood_overview-2.pdf}
    \caption{\textbf{Training pipeline for {\sc mirkwood} in five sequential steps.} %In what follows, we refer to the test subset -- for which we desire to obtain predictions -- as $\mathcal{D_{TEST}}$; the training subset -- on which the \textsc{NGBoost} algorithm is trained -- as $\mathcal{D_{TRAIN}}$; and the input data set consisting of both of these as $\mathcal{D}$. Given a sample of galaxy flux values as input, a `prediction' consists of a mean ($\mu$) and a standard deviation ($\sigma$) for the desired galaxy property. 
    \emph{\textbf{Step 1:}} We divide the input data set $\mathcal{D}$ into $N_{\rm CV,1} = 4$ cross-validation folds, at any point referring to the collation of $N_{\rm CV,1}-1$ of them as $\mathcal{D_{TRAIN}}$, and the remaining fold as $\mathcal{D_{TEST}}$. We repeat this $N_{\rm CV,1}$ times to cover all samples in $\mathcal{D}$, but depict only one such iteration here for illustration. \emph{\textbf{Step 2:}} We sub-divide $\mathcal{D_{TRAIN}}$ into $N_{\rm CV,2} = 3$ CV folds. Same as before, $N_{\rm CV,2}-1$ folds are collated while the remaining fold, referred to as the validation set $\mathcal{V}$, is set aside. \emph{\textbf{Step 3:}} Each of the $N_{\rm CV,2}$ CV folds is used to create $N_{\rm bags} = 3$ `bags' by randomly shuffling its data and picking the same number of samples with replacement. An \textsc{NGBoost} model with a given set of hyperparameters is copied over $N_{\rm bags}$ times, and each copy is trained on one `bag' of data. The predictions of all $N_{\rm bags}$ models on $\mathcal{V}$ are recorded and averaged according to Equation \ref{eqn:main_averaging_eqn} to obtain the mean, epistemic, and aleatoric uncertainties for $\mathcal{V}$. \emph{\textbf{Step 4:}} This process is repeated 100 times to find better performing hyperparameters for \textsc{NGBoost}; we refer to thus optimized model as {\sc NGBoost$_{\rm{OPT}}$}. \emph{\textbf{Step 5:}} Finally, we train {\sc NGBoost$_{\rm{OPT}}$} on $\mathcal{D_{TRAIN}}$ and predict the output for $\mathcal{D_{TEST}}$.} %the predictions on $\mathcal{V}$ are used to \emph{post hoc} modify the predictions on $\mathcal{D_{TEST}}$ as described in Section ().}
    \label{fig:mirkwood_pipeline}
\end{figure*}

We now present implementation details of our proposed method. {\sc mirkwood} is a \emph{supervised} learning algorithm, meaning it requires a \emph{training set} consisting of a pairs of inputs and outputs, to be able to learn the mapping from the former to the latter. Each input consists of a set of discrete \emph{features}, or independent variables, whereas the outputs -- also referred to as \emph{labels} -- are the dependent variables. The algorithm learns this mapping by minimizing a user-specified \emph{loss function} -- think minimization of the mean squared error commonly employed when fitting data in linear regression analysis. In this work, each input $\mathbf{x}$ is a mock SED vector consisting of flux values in 35 bands, and the associated galaxy properties (redshift, stellar mass, dust mass, stellar metallicity, and instantaneous star formation rate) form a vector output of length 5. While certain types of ML algorithms are able to map each input vector to an output vector consisting of multiple labels (for example, neural networks), this is not possible with {\sc mirkwood}. Hence we associate with each input only one galaxy property at a time, and use the model five times. Let us denote by $\mathbf{x}$ an input SED vector, by $y$ a galaxy property, by $n$ the number of SED samples, and by $d$ the number of bands/filters. Then the data set on hand can be mathematically specified as $\mathcal{D}=\left\{\left(\mathbf{x}_{i}^{1:d}, y_{i}\right): i=1, \ldots, n\right\}$. Our aim is to learn a data-driven mapping from the set of all $\mathbf{x}_{i}$s to the set of all $ y_i$s, to be able to predict $y_\mathrm{new}$ for a new, unseen observation $\mathbf{x_\mathrm{new}}$. To solve this \emph{regression} problem\footnote{Classification tasks are those where the goal is to predict discrete labels, e.g. identifying whether an animal is a cat or a dog. In regression problems we aim to prediction continuous labels, e.g. predicting the price of a stock tomorrow given its price over the past year.}, we employ the \textsc{NGBoost} algorithm \citep{ngboost}. Unlike most commonly used ML algorithms and libraries such as Random Forests \citep{randomforests}, Randomized Trees \citep{extremelyrandomizedtrees}, XGBoost \citep{xgboost} and Gradient Boosting Machines \citep{lightgbm}, \textsc{NGBoost} enables us to easily work in a probabilistic setting, and corresponding to every input galaxy SED, output both a measure of the central tendency (i.e. $\mu$), and a measure of dispersion (i.e. $\sigma$) for the galaxy property of interest. We thus use {\sc NGBoost} as the backbone of {\sc mirkwood}, and use the hyper-parameters suggested by \cite{ren2019rongba_ngboost}\footnote{\cite{ren2019rongba_ngboost} found that their new set of hyperparameters result in faster convergence than the default values supplied by the developers at \url{https://github.com/stanfordmlgroup/ngboost/blob/master/ngboost/ngboost.py}.}. We make the assumption that samples are drawn from Gaussian distributions. % therefore its probability density function is given by $\mathrm{PDF}(y_i) = (2\pi \sigma_{\rm a}^2)^{-1/2} \exp{\frac{-(y_i - \mu)}{\sigma_{\rm a}^2}}\mathcal{N}$
Our loss function is the \emph{negative likelihood function} \citep{ngboost}.

Consider the case where we have samples from all three simulations. At z=0, we have 1,797 samples from {\sc Simba}, 4,697 from {\sc Eagle}, and 10,073 from {\sc IllustrisTNG}. The corresponding figures at z=2 are 1,961, 5,734 and 9,324. To predict the galaxy property under consideration for each of these ($n=33,586$) galaxies, we proceed as follows. First, we fix the parameters of the {\sc NGBoost} model to those recommended by \cite{ren2019rongba_ngboost}. Then, we divide the $n$ samples into $N_{\rm{CV,1}}=5$ distinct subsets (or \emph{folds}) based on \emph{stratified sampling} -- $y_i$s in each subset are picked such that their distribution closely matches the distribution of the parent sample $y_i$s. The first four subsets taken together form the \emph{training set}, $\mathcal{D_{TRAIN}}$, while the fifth, left-out fold for which we assume output labels are unavailable, is called the \emph{test set}, $\mathcal{D_{TEST}}$. This is the first step show in Figure \ref{fig:mirkwood_pipeline}. We then sub-divide $\mathcal{D_{TRAIN}}$ into $N_{\rm{CV,2}} = 5$ subsets, again in a stratified fashion. The model is trained cyclically on the combination of any distinct four sub-subsets -- referred to as $\mathcal{D_{TRAIN_{TRAIN}}}$, while its predictions on the samples in the left-out sub-subset, $\mathcal{D_{TRAIN_{VAL}}}$, are recorded and stored. Instead of training directly on $\mathcal{D_{TRAIN_{TRAIN}}}$, we use create  $N_{\rm bags} = 48$ `bags' by randomly shuffling the data and picking the same number of samples \emph{with replacement}. The {\sc NGBoost} model initialized earlier is trained on all bags, and the respective predictions on  $\mathcal{D_{TRAIN_{VAL}}}$ are averaged. The exact method of averaging is expounded upon in Section \ref{sec:methods_uncertainty}. After $N_{\rm{CV,2}}$ rounds we have $N_{\rm{CV,2}}$ non-overlapping $\mathcal{D_{TRAIN_{VAL}}}$ data sets containing distinct samples, which taken together constitute $\mathcal{D_{TRAIN}}$. These together constitute the second and third steps in the pipeline. For each of the 26,869 samples, we compare the predicted galaxy properties with their ground truth values, and note the average negative-log likelihood, $\mathcal{NLL_{\rm{VAL}}}$. We repeat this exercise multiple times, on each iteration tuning {\sc NGBoost}'s hyperparameters so that the $\mathcal{NLL_{\rm{VAL}}}$ is as low as possible. With the optimized set of {\sc NGBoost} hyperparameters thus obtained, we train {\sc mirkwood} on the entire training set $\mathcal{D_{TRAIN}}$, and record its predictions on $\mathcal{D_{TEST}}$. This process of \emph{hyperparameter optimization} is the fourth step in the pipeline. Finally, this process is repeated $N_{\rm{CV,1}}-1$ more times, to obtain predictions on all $n$ samples -- this is the fifth and final step in the pipeline. The entire process is carried out in a \emph{chained} fashion -- the model is first trained to use galaxy flux values to predict redshift, then the predicted redshifts in conjunction with the original flux values are used to predict galaxy stellar mass, and so on; this is explained pictorially in Figure \ref{fig:chaining}. We know that galaxy properties can be strongly degenerate (for instance, the well-known age-dust-metallicty degeneracy); by chaining, we `hack' our model to leverage the inter-dependencies between these parameters. To predict SFR$_{100}$, the galaxy SFR average over the last 100 Myr, for an unseen sample $x_{\textrm{new}}$, for instance, we will use \textsc{NGBoost} %the model that was trained on samples split stratifically based on SFR$_{100}$, and
to first predict galaxy redshift, galaxy stellar mass, then galaxy dust mass, then stellar metallicity, and finally SFR$_{100}$.


==> shap_clustering.tex <==
\subsection{SHAP Clustering}\label{sec:shap_clustering}
You can cluster your data with the help of Shapley values. The goal of clustering is to find groups of similar instances. Normally, clustering is based on features. Features are often on different scales. For example, height might be measured in meters, color intensity from 0 to 100 and some sensor output between -1 and 1. The difficulty is to compute distances between instances with such different, non-comparable features.

SHAP clustering works by clustering on Shapley values of each instance. This means that you cluster instances by explanation similarity. All SHAP values have the same unit -- the unit of the prediction space. You can use any clustering method. The following example uses hierarchical agglomerative clustering to order the instances.

The plot consists of many force plots, each of which explains the prediction of an instance. We rotate the force plots vertically and place them side by side according to their clustering similarity.


==> shap_decision_plots.tex <==
\subsection{SHAP Decision Plots}
%https://towardsdatascience.com/explain-your-model-with-the-shap-values-bc36aac4de3d
Let me describe this elegant plot in great detail: The output value is the prediction for that observation (the prediction of the first row in Table B is 6.20). The base value: The original paper explains that the base value E(y$_{hat}$) is `the value that would be predicted if we did not know any features for the current output.' In other words, it is the mean prediction, or mean(yhat). You may wonder why it is 5.62. This is because the mean prediction of Y$_{test}$ is 5.62. You can test it out by Y$_{test}$.mean() which produces 5.62.
Red/blue: Features that push the prediction higher (to the right) are shown in red, and those pushing the prediction lower are in blue.
Alcohol: has a positive impact on the quality rating. The alcohol content of this wine is 11.8 (as shown in the first row of Table B) which is higher than the average value 10.41. So it pushes the prediction to the right.
pH: has a negative impact on the quality rating. A lower than the average pH (=3.26 < 3.30) drives the prediction to the right.
Sulphates: is positively related to the quality rating. A lower than the average Sulphates (= 0.64 < 0.65) pushes the prediction to the left.

\iffalse
You may wonder how we know the average values of the predictors. Remember the SHAP model is built on the training data set. The means of the variables are: X$_$train.mean()

X$_$train.mean()
What is the result for the 2nd observation in Table B look like? Let's doshap_plot(1):

How about the 3rd observation in Table B? Let’s do shap_plot(2):

Just to do one more before you become bored. The 4th observation in Table B is this: shap_plot(3)
\fi

==> shap_dependence_plot.tex <==
\subsection{SHAP Dependence Plot}\label{sec:shap_dep_plot}
SHAP dependence plots show how a feature’s value (x-axis) impacted the prediction (y-axis) of every sample (each dot)
in a dataset (Figures 4B and E; Methods 15). This provides richer information than traditional partial dependence
plots (Supplemental Figure 8). For the mortality model this reproduces the standard risk inflection point of systolic
blood pressure [23], while also highlighting that the impact of blood pressure risk is different for people of different
ages (Figure 4B). Many individuals have a recorded blood pressure of 180 mmHg in the mortality dataset, but the
impact of that measurement on their mortality risk varies because early onset high blood pressure is more concerning
to the model than late onset high blood pressure. These types of interaction effects show up as vertical dispersion in
SHAP dependence plots.
For the chronic kidney disease model, a dependence plot again clearly reveals a risk inflection point for systolic
blood pressure, but in this dataset the vertical dispersion from interaction effects appears to be partially driven by
differences in blood urea nitrogen (Figure 4E). Correctly modeling blood pressure risk while retaining interpretabilty
is important since blood pressure control in select chronic kidney disease (CKD) populations may delay progression of
kidney disease and reduce the risk of cardiovascular events (Methods 15).


SHAP dependence plots show the effect of a single feature across the whole dataset. They plot a feature's value v/s. the SHAP value of that feature across many samples. SHAP dependence plots are similar to partial dependence plots, but account for the interaction effects present in the features, and are only defined in regions of the input space supported by data. The vertical dispersion of SHAP values at a single feature value is driven by interaction effects, and another feature is chosen for coloring to highlight possible interactions. Figure () (described in more detail in \S\ref{sec:results}) shows the dependence plots for 

While a SHAP summary plot gives a general overview of each feature a SHAP dependence plot show how the model output varies by feauture value. Note that every dot is a person, and the vertical dispersion at a single feature value results from interaction effects in the model. The feature used for coloring is automatically chosen to highlight what might be driving these interactions. Later we will see how to check that the interaction is really in the model with SHAP interaction values. Note that the row of a SHAP summary plot results from projecting the points of a SHAP dependence plot onto the y-axis, then recoloring by the feature itself.

SHAP feature dependence might be the simplest global interpretation plot: 1) Pick a feature. 2) For each data instance, plot a point with the feature value on the x-axis and the corresponding Shapley value on the y-axis. 3) Done.

Mathematically, the plot contains the following points:  
$\left\{\left(x_{j}^{(i)}, \phi_{j}^{(i)}\right)\right\}_{i=1}^{n}$

The following figure shows the SHAP feature dependence for years on hormonal contraceptives:

SHAP dependence plots are an alternative to partial dependence plots and accumulated local effects. While PDP and ALE plot show average effects, SHAP dependence also shows the variance on the y-axis. Especially in case of interactions, the SHAP dependence plot will be much more dispersed in the y-axis. The dependence plot can be improved by highlighting these feature interactions.


==> shap_summary_plots.tex <==
\subsection{SHAP Summary Plots}\label{sec:shap_summary}
\iffalse
Combining local explanations from TreeExplainer across an entire dataset enhances traditional global representations
of feature importance by: 1) avoiding the inconsistency problems of current methods (Supplementary Figure 2), 2)
increasing the power to detect true feature dependencies in a dataset (Supplementary Figure 7), and 3) enabling us
to build SHAP summary plots that succinctly display the magnitude, prevalence, and direction of a feature’s effect.
SHAP summary plots avoid conflating the magnitude and prevalence of an effect into a single number, and so reveal
rare high magnitude effects. Figure 4A illustrates its benefits using the mortality dataset: (left) a standard bar-chart
based on the average magnitude of the SHAP values, and (right) a set of beeswarm plots where each dot corresponds
to an individual person in the study. The position of the dot on the x-axis is the impact that feature has on the
model’s prediction for that person. When multiple dots land at the same x position they pile up to show density.
Figure 4A (right) reveals the direction of effects, such as men (blue) having a higher mortality risk than women
(red); and the distribution of effect sizes, such as the long right tails of many medical test values. These long tails
mean features with a low global importance can yet be extremely important for specific individuals. Interestingly, rare
mortality effects always stretch to the right, which implies there are many ways to die abnormally early when medical
measurements are out-of-range, but not many ways to live abnormally longer (Methods 14).
\fi

The \emph{SHAP summary plot} is a graphical way of succinctly displaying the \emph{magnitude}, \emph{prevalence}, and \emph{direction} of a feature's effect. It is an extension of the standard bar-chart based on the average magnitude of the SHAP values, and simultaneously displays both feature importance with feature effects.% Each point on the summary plot is a Shapley value for a feature and an instance.
The position on the x-axis is determined by the feature and on the y-axis by the Shapley value. The color represents the value of the feature from low to high. Overlapping points are jittered in y-axis direction, so we get a sense of the distribution of the Shapley values per feature. The features are ordered according to their importance. We consider the case of predicting galaxy mass, and show the resulting bar plot and the summary plot in Figure (). As is apparent, the summary plot is a high resolution version of the bar plot, which shows the \emph{global} relationship between the value of a feature and the impact on the prediction. But to see the exact form of the relationship, we have to look at SHAP dependence plots.

\iffalse
%%%% Chained vs Unchained, SHAP. %%%%%%%
\begin{figure*}
\gridline{\fig{images/Mass_shap_chain_ngb.eps}{0.28\textwidth}{(a)}
          }
\gridline{\leftfig{images/Dust Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Metallicity_shap_chain_ngb.eps}{0.28\textwidth}{(b)}
          \rightfig{images/Star Formation Rate_shap_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Dust Mass_shap_ngb.eps}{0.28\textwidth}{}
          \fig{images/Metallicity_shap_ngb.eps}{0.28\textwidth}{(c)}
          \rightfig{images/Star Formation Rate_shap_ngb.eps}{0.28\textwidth}{}
          }
\caption{Inverted pyramid figure of six individual files. The nova are (a) V2491 Cyg, (b) HV Cet, (c) LMC 2009, (d) RS Oph, (e) U Sco, and (f) KT Eri. These individual figures are taken from
\label{fig:shap_chainedvsunchained}}
\end{figure*}

%%%% Chained vs Unchained Scatter
\begin{figure*}
\gridline{\fig{images/Mass_scatter_chain_ngb.eps}{0.3\textwidth}{(a)}
          }
\gridline{\leftfig{images/Dust Mass_scatter_chain_ngb.eps}{0.3\textwidth}{}
          \fig{images/Metallicity_scatter_chain_ngb.eps}{0.3\textwidth}{(b)}
          \rightfig{images/Star Formation Rate_scatter_chain_ngb.eps}{0.3\textwidth}{}
          }
\gridline{\leftfig{images/Dust Mass_scatter_ngb.eps}{0.3\textwidth}{}
          \fig{images/Metallicity_scatter_ngb.eps}{0.3\textwidth}{(c)}
          \rightfig{images/Star Formation Rate_scatter_ngb.eps}{0.3\textwidth}{}
          }
\caption{We also highlight the importance of chaining models to account for dependenceFor each of the seven subplots, values predicted by mirkwood are plotted on the y-axis, while ground-truth values are on the x-axis. \textbf{(a):} Galaxy mass, in units of M$_{\odot}$. \textbf{(b):} From left to right: dust mass in units of M$_{\odot}$, gas phase metallicity in units of solar metallicity, and star formation rate in units of $\frac{M_{\odot}}{\textrm{year}}$. \textbf{(c):}}
\label{fig:scatter_chainedvsunchained}
\end{figure*}

%%% Chained scatter, effect of noise
\begin{figure*}
\gridline{\leftfig{images/Mass_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Mass_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Mass_scatter_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Dust Mass_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Dust Mass_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Dust Mass_scatter_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Metallicity_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Metallicity_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Metallicity_scatter_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Star Formation Rate_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Star Formation Rate_scatter_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Star Formation Rate_scatter_chain_ngb.eps}{0.28\textwidth}{}
          }
\caption{effect of noise}
\label{fig:scatter_chained_effectofnoise}
\end{figure*}

%%% Chained SHAP, effect of noise
\begin{figure*}
\gridline{\leftfig{images/Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Dust Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Dust Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Dust Mass_shap_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Metallicity_shap_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Metallicity_shap_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Metallicity_shap_chain_ngb.eps}{0.28\textwidth}{}
          }
\gridline{\leftfig{images/Star Formation Rate_shap_chain_ngb.eps}{0.28\textwidth}{}
          \fig{images/Star Formation Rate_shap_chain_ngb.eps}{0.28\textwidth}{}
          \rightfig{images/Star Formation Rate_shap_chain_ngb.eps}{0.28\textwidth}{}
          }
\caption{effect of noise}
\label{fig:shap_chained_effectofnoise}
\end{figure*}
\fi

\iffalse
\begin{figure*}
\begin{multicols}{2}
    \includegraphics[width=.9\linewidth]{images/logmass_shap_chain_ngb.eps}\par 
    \includegraphics[width=.9\linewidth]{images/logdustmass_shap_chain_ngb.eps}\par 
\end{multicols}
\begin{multicols}{2}
    \includegraphics[width=.9\linewidth]{images/logmet_shap_chain_ngb.pdf}\par
    \includegraphics[width=.9\linewidth]{images/logsfr_shap_chain_ngb.pdf}\par
\end{multicols}
\caption{abc}
\label{fig:fig9}
\end{figure*}
\fi


==> uncertainty_quantification.tex <==
\subsection{Uncertainty Quantification}\label{sec:methods_uncertainty}
Real observations differ from simulations in a number of ways.
\begin{itemize}
    \item It is rarely the case that as observers we have access to all filters in a survey for every observed galaxy. For example, we might encounter a situation where we are interested in determining a galaxy's mass from its photometry, but do not have access to $K$ and $H$ band information, thus making our task difficult.
    \item Different filters have differing sensitivities and noise properties, resulting in non-uniform measurement noises across observation bands. Even in an ideal case where observations in UV, optical and IR are equally robust, there is an irreducible Poisson measurement error.
    \item While modern hydrodynamical simulations, such as those used in this work, are powerful modellers of the known Universe, they are nonetheless just that -- models. There is an inherent, irreducible \emph{domain gap} between our approximation of reality, and reality. Imperfect modeling assumptions both about known physical processes, and arising from our sheer lack of knowledge of them, are primary contributors to this gap. Some specific reasons are modeling star formation with a sub-resolution model, divergence of modeled stellar mass functions from observed ones, and incomplete understanding of AGN feedback processes.
    \item Any supervised ML algorithm is only as good as the data on which it is trained. It might well be the case that an observed galaxy is in a completely different parameter space than any of the galaxies in our training set. %For example, in Figure () we consider the case where \textsc{mirkwood} is trained on only \textsc{Simba} galaxies, and is asked to predict stellar mass for galaxies in \textsc{Eagle} and \textsc{IllustrisTNG}. As can be seen, the model performance is severely lacking in the non-overlapping part of the histograms in Figure ()(). 
    \item Even if some particular model, say \textsc{NGBoost}, with a given set of hyperparameters, is able to faithfully and satisfactorily predict galaxy properties, it is very well possible that there exist other models which can also make predictions that are just as accurate. It is also possible that for our chosen model/set of models, a different data pre-processing scheme, choice of hyperparameters (as mentioned in Section \ref{sec:methods_proposed_method}, the chosen set of hyperparameters is locally optimal but is not guaranteed to be globally optimal), or choice of scheme for balancing classes might result in better predictions.
\end{itemize}

Owing to these factors, a highly desirable behavior of any predictive model would be to not only return a point prediction (per galaxy property under consideration), but also some quantity conveying the model's belief or confidence in its output \citep{kendall2017uncertainties, choi2018uncertainty}. We can break down such \emph{predictive uncertainty} into two parts--\emph{aleatoric} and \emph{epistemic}  \cite{kendall2017uncertainties}\footnote{The word epistemic comes from the Greek ``episteme", meaning ``knowledge"; epistemic uncertainty is ``knowledge uncertainty". Aleatoric comes from the Latin ``aleator", meaning ``dice player"; aleatoric uncertainty is the ``dice player's" uncertainty \citep{gal_thesis}}. Aleatoric uncertainty captures the uncertainty in the data generating process -- for example, measurement noise in filters, or the inherent randomness of a coin flipping experiment. It cannot be reduced by collecting more training data\footnote{We know that a fair coin has a 0.5 probability of landing heads, yet we cannot assert with 100\% certainty the outcome of the next flip, no matter how many times we have already flipped the coin.}; however, it can be reduced by collecting more informative features\footnote{Uncertainty in galaxy mass estimation in the absence of H and K band information can be drastically reduced by collecting high quality data in these bands.}. On the other hand, epistemic uncertainty models the ignorance of the predictive model, and can indeed be explained away given a sufficiently large training dataset\footnote{If we are given a biased coin where we do not know the probability $p$ of turning up heads, we can determine it to arbitrary precision by flipping the coin an arbitrarily large number of times and counting the number of times it turns up heads.}. Aleatoric uncertainty is thus \emph{irreducible} or \emph{statistical}, epistemic being its \emph{reducible} or \emph{systematic} cousin. Aleatoric uncertainty covers first three of the five issues above, while epistemic uncertainty subsumes the last two points. High aleatoric uncertainty can be indicative of noisy measurements or missing informative features, while high epistemic uncertainty could be a clue that the observed galaxy is very different that any of the galaxies the model was trained on (such a galaxy is referred to as being \emph{out of distribution}).

As previously discussed, the aim for a supervised ML algorithm is to learn the latent data generating mechanism that maps each input sample $\mathbf{x}_{i}$ to its corresponding output label $y_{i}$. This can be represented as follows:%We compute probability density function for every input. Here we
\[
y_i=f(\mathbf{x}_i)+\eta_{i}
\]
where $f(\cdot)$ is the \emph{unknown} latent function and a measurement error $\eta$ follows a standard normal distributions distribution with a variance $\sigma_{\eta,i}^{2},$ i.e., $\eta_i \sim \mathcal{N}\left(\mu=0, \sigma_{\eta,i}^{2}\right)$. The variance of $\eta_i$ corresponds to the aleatoric uncertainty, i.e., $\sigma_{\eta,i}^{2}=\sigma_{a,i}^{2}$ where we will denote $\sigma_{a,i}^{2}$ as aleatoric uncertainty associated with the observation $\mathbf{x}_{i}$. Similarly, epistemic uncertainty will be denoted as $\sigma_{e,i}^{2}$. Since $f(\cdot)$ is unknown, by training on the \emph{training set} the model attempts to approximate, or guess, this function as closely as possible. Suppose that we train $\hat{f}(\mathbf{x})$ to approximate $f(\mathbf{x})$ from the samples in the input data set, $\mathcal{D}$. Then, we can see that
%\[
%\sigma_{e}^{2}=\mathbb{E}\|f(\mathbf{x})-\hat{f}(\mathbf{x})\|^{2}
%\]
%Then, we can see that
\[
\begin{aligned}
\mathbb{E}\|y_i-\hat{f}(\mathbf{x}_i)\|^{2} &=\mathbb{E}\|y_i-f(\mathbf{x}_i)+f(\mathbf{x}_i)-\hat{f}(\mathbf{x}_i)\|^{2} \\
&=\mathbb{E}\|y_i-f(\mathbf{x}_i)\|^{2}+\mathbb{E}\|f(\mathbf{x}_i)-\hat{f}(\mathbf{x}_i)\|^{2} \\
&=\sigma_{a,i}^{2}+\sigma_{e,i}^{2},
\end{aligned}
\]
where $\mathbb{E}\|\cdot\|$ is the expectation operator. This indicates the total predictive variance is the sum of aleatoric uncertainty and epistemic uncertainty.

%In this work, we pre-process each of the four galaxy properties to a normal form: we center by removing their respective medians, and scale by their respective interquartile range\footnote{Specifically, we use the \textsc{RobustScaler} function from the popular ML package \textsc{scikit-learn} in \textsc{Python}.}.  %\citep{yeo_johnson_pt}.
%This allows us to use the `normal' distribution in \textsc{NGBoost}, obtaining a mean and a standard deviation for every SED, per \emph{output label} (galaxy property). 

The \textsc{NGBoost} algorithm that forms the backbone of {\sc mirkwood} is naturally able to output both the mean $\mu_i$ and the aleatoric uncertainty $\sigma_{a,i}^2$ for a given observation $\mathbf{x}_i$. To obtain the epistemic uncertainty $\sigma_{e,i}^2$, we use \emph{bootstrapping}. This involves creating multiples copies of the same training dataset, each time picking samples \emph{with replacement}, training the same model on all copies, and averaging the results. The goal is to simulate a scenario where a model only has access to limited samples -- and hence limited parameter space -- and to study how this impacts its predictive ability (see Figure \ref{fig:mirkwood_pipeline}, especially \emph{\textbf{Step 3}}). That is, given an \textsc{NGBoost} model, the predicted label for an observation $\mathbf{x}_{i}$ is represented as:
\begin{align*}
p(\mathbf{y} \mid \mathbf{x}_{i}) &= \mathcal{N}\left(\mu_{i}, \sigma_{a,i}^2\right),
\end{align*}

Creating $N_{\rm bags}$ bootstrapped bags essentially creates $N_{\rm bags}$ copies of the above equation. To obtain final summary statistics, we combine them as
\begin{align}
\hat{\mu}_i {=}\sum_{j=1}^{N_{\rm bags}}\mu_{i,j};\;\hat{\sigma}_{i,a}^2 {=} \sum_{j=1}^{N_{\rm bags}} \sigma_{i,a,j}^{2};\;\hat{\sigma}_{i,e}^2 {=} \sum_{j=1}^{N_{\rm bags}} (\mu_{i,j} {-} \hat{\mu}_i)^2
\label{eqn:main_averaging_eqn}
\end{align}

The upshot of this exercise is that the errors modeled by {\sc mirkwood} encapsulates both the propagated noise due in the input samples, and the uncertainty arising due to the finite size of the training set. Neither {\sc Prospector} nor previous projects in this field \citep{lovell2019learning,acquaviva2015simultaneous} take into account this latter source of uncertainty. This is a significant contribution of {\sc mirkwood} and helps mitigate the over-confidence in predictions that is typical of machine learning models.
%\begin{equation*}
%\mathbb{V}(y \mid \mathbf{x}) \approx \frac{1}{T} \sum_{t=1}^{T} \hat{\mu}_{t}^{2}(\mathbf{x})-\left(\sum_{t=1}^{T} \hat{\mu}_{t}(\mathbf{x})\right)^{2}+\frac{1}{T} \sum_{t=1}^{T} \hat{\sigma}(\mathbf{x})
%\end{equation*}

%Correctly acquiring and distinguishing each type of uncertainty is important to many practical problems. Suppose that we are making our model to predict the steering angle of an autonomous driving car (which is exactly the case in our experiments) where the training data is collected from human drivers with an accurate measurement device. In this case, high aleatoric uncertainty and small epistemic uncertainty indicate that there exist multiple possible steering angles. For example, a driver can reasonably steer the car to both left and right in case of another car in front and both sides open. However, when the prediction has low aleatoric uncertainty and high epistemic uncertainty, this indicates that our model is uncertain about the current prediction which could possibly due to the lack of training data. In this case, it is reasonable to switch to a risk-averse controller or alarm the driver, if possible. Epistemic and aleatoric uncertainties are sometimes referred to as reducible and irreducible uncertainties respectively, since epistemic uncertainty can be reduced with more data (knowledge), while aleatoric uncertainty cannot (the stochasticity of a dice roll cannot be reduced by observing more rolls).


\begin{table*}
    \caption{Summary of machine learning terms and variables appearing in this work.}
    \label{tab:meaningsofterms}
    \centering
    \begin{tabular}{p{0.15\linewidth} p{0.80\linewidth}}
    \toprule
    Term & Meaning \\ \tableline
    \emph{Bagging} & Bootstrapped Aggregation. A machine learning meta-algorithm that generates $N_{\rm bags}$ new training sets by sampling from the parent training data set uniformly and with replacement. Each bag may or may not be the same size as the parent training data set. \\ 
    \emph{HPO} & Hyperparameter optimization. The task of finding a well performing set of hyperparameters for any given ML algorithm. \\
    \emph{Chaining} & Given multiple outputs of interest (dependent variables), the technique of running the regression model in sequence to exploit correlations among them. \\
    \emph{Cross validation} & The task of dividing the training set into non-overlapping `folds' for the purpose of hyperparameter optimization. \\
    $\mathcal{D}$ & Input training set comprising of all samples from {\sc Simba}, {\sc Eagle}, and {\sc IllustrisTNG}. Each sample consists of input (independent variables)-output(dependent variables) pairs.  \\
    $\mathcal{D_{TRAIN}}$ & Training set, derived from $\mathcal{D}$. {\sc mirkwood} is trained on this, and used for inference on $\mathcal{D_{TEST}}$. \\
    $\mathcal{D_{TRAIN_{TRAIN}}}$ & Training set, derived from $\mathcal{D_{TRAIN}}$. Used for HPO. \\
    $\mathcal{D_{TRAIN_{VAL}}}$ & Validation set, derived from $\mathcal{D_{TRAIN}}$. Used for HPO. \\
    $\mathcal{D_{TEST}}$ & Test set. \\ 
    $N_{\rm{CV,1}}$ & Number of CV folds that is used to produce $\mathcal{D_{TRAIN}}$ and $\mathcal{D_{TEST}}$ from $\mathcal{D}$. \\
    $N_{\rm{CV,2}}$ & Number of CV folds that is used to produce $\mathcal{D_{TRAIN_{TRAIN}}}$ and $\mathcal{D_{TRAIN_{VAL}}}$ from $\mathcal{D_{TRAIN}}$. \\
    $\sigma_{e}$ & Epistemic uncertainty. \\
    $\sigma_{a}$ & Aleatoric uncertainty. \\
    $f(\cdot)$ & Functional representation of {\sc mirkwood}. This acts on a given input vector $\mathbf{x}$ to produce the output $y$. \\
    $\mu$ & The mean of a predicted galaxy property, using one bag of training data. \\
    $\hat{\mu}$ & The mean of $\mu$s predicted by all $N_{\rm{bags}}$ bags. \\ \tableline
    \end{tabular}
\end{table*}

